Hyper-parameter Tuning for Adversarially Robust Models

This work focuses on the problem of hyper-parameter tuning (HPT) for robust (i.e., adversarially trained) models, shedding light on the new challenges and opportunities arising during the HPT process for robust models. To this end, we conduct an extensive experimental study based on 3 popular deep models, in which we explore exhaustively 9 (discretized) HPs, 2 fidelity dimensions, and 2 attack bounds, for a total of 19208 configurations (corresponding to 50 thousand GPU hours). Through this study, we show that the complexity of the HPT problem is further exacerbated in adversarial settings due to the need to independently tune the HPs used during standard and adversarial training: succeeding in doing so (i.e., adopting different HP settings in both phases) can lead to a reduction of up to 80% and 43% of the error for clean and adversarial inputs, respectively. On the other hand, we also identify new opportunities to reduce the cost of HPT for robust models. Specifically, we propose to leverage cheap adversarial training methods to obtain inexpensive, yet highly correlated, estimations of the quality achievable using state-of-the-art methods. We show that, by exploiting this novel idea in conjunction with a recent multi-fidelity optimizer (taKG), the efficiency of the HPT process can be enhanced by up to 2.1x.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> plots/correlations.tex <==


\if0
\begin{figure*}[t]
\centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{plots/imageNet/imageNet_epochs_epsilon_acc.pdf}
        \caption{ResNet50 with ImageNet}
        \label{fig:bound_acc_imagenet}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{plots/cifar10/cifar10_epochs_epsilon_acc.pdf}
        \caption{CNN with Cifar10}
        \label{fig:bound_acc_cifar10}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{plots/mnist/mnist_epochs_epsilon_acc.pdf}
        \caption{CNN with MNIST}
        \label{fig:bound_acc_mnist}
    \end{subfigure}

    \caption{Standard and adversarial error of the optimal configurations using different bounds $\epsilon$ to train different models and benchmarks. Continuous and dashed lines correspond to standard and  adversarial error, respectively.}
     \label{fig:bound_acc}
\end{figure*}
\fi









\begin{figure*}[t]
\centering
    \captionsetup{justification=centering,}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[ width=\textwidth]{plots/imageNet/imageNet_epochs_correlation_2.0.pdf}
        \caption{Error Corr. \\ResNet50/ImageNet $\epsilon$\textdblhyphen2}
        \label{fig:correlation_acc_imageNet_2}
    \end{subfigure}\hspace{2mm}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{plots/imageNet/imageNet_epochs_correlation_AdvAcc_2.0.pdf}
        \caption{Adv. Error Corr. \\ResNet50/ImageNet $\epsilon$\textdblhyphen2}
        \label{fig:correlation_advacc_imageNet_2}
    \end{subfigure}\hspace{2mm}    
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[ width=\textwidth]{plots/imageNet/imageNet_epochs_cdfCosts.pdf}
        \caption{CDF time reduction  \\ResNet50/ImageNet}
        \label{fig:cost_imageNet}
    \end{subfigure}
\if0
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{plots/imageNet/imageNet_epochs_correlation_4.0.pdf}
        \caption{Error Corr. ResNet50/ImageNet $\epsilon$\textdblhyphen4}
        \label{fig:correlation_acc_imageNet_4}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[  width=\textwidth]{plots/imageNet/imageNet_epochs_correlation_AdvAcc_4.0.pdf}
        \caption{Adv. Error Corr. ResNet50/ImageNet $\epsilon$\textdblhyphen4}
        \label{fig:correlation_advacc_imageNet_4}
    \end{subfigure}
\fi

\vspace{3mm}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[ width=\textwidth]{plots/svhn/svhn_epochs_correlation_4.0.pdf}
        \caption{Error Corr. \\ResNet18/SVHN $\epsilon$\textdblhyphen4}
        \label{fig:correlation_acc_svhn_4}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{plots/svhn/svhn_epochs_correlation_AdvAcc_4.0.pdf}
        \caption{Adv. Error Corr. \\ResNet18/SVHN $\epsilon$\textdblhyphen4}
        \label{fig:correlation_advacc_svhn_4}
    \end{subfigure}  
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[ width=\textwidth]{plots/svhn/svhn_epochs_correlation_8.0.pdf}
        \caption{Error Corr. \\ResNet18/SVHN $\epsilon$\textdblhyphen8}
        \label{fig:correlation_acc_svhn_8}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[ width=\textwidth]{plots/svhn/svhn_epochs_correlation_AdvAcc_8.0.pdf}
        \caption{Adv. Error Corr. \\ResNet18/SVHN $\epsilon$\textdblhyphen8}
        \label{fig:correlation_advacc_svhn_8}
    \end{subfigure}
    
\vspace{3mm}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[ width=\textwidth]{plots/cifar10/cifar10_epochs_correlation_8.0.pdf}
        \caption{Error Corr. \\CNN/Cifar10 $\epsilon$\textdblhyphen8}
        \label{fig:correlation_acc_cifar10_8}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[ width=\textwidth]{plots/cifar10/cifar10_epochs_correlation_AdvAcc_8.0.pdf}
        \caption{Adv. Error Corr. \\CNN/Cifar10 $\epsilon$\textdblhyphen8}
        \label{fig:correlation_advacc_cifar10_8}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[ width=\textwidth]{plots/cifar10/cifar10_epochs_correlation_12.0.pdf}
        \caption{Error Corr. \\CNN/Cifar10 $\epsilon$\textdblhyphen12}
        \label{fig:correlation_acc_cifar10_12}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[ width=\textwidth]{plots/cifar10/cifar10_epochs_correlation_AdvAcc_12.0.pdf}
        \caption{Adv. Error Corr. \\CNN/Cifar10 $\epsilon$\textdblhyphen12}
        \label{fig:correlation_advacc_cifar10_12}
    \end{subfigure}
    

    %\begin{subfigure}[b]{0.24\textwidth}
    %    \includegraphics[  trim=1mm 2mm 2.3cm 2.3cm clip, width=\textwidth]{plots/cifar10/cifar10_epochs_cdfCosts.pdf}
    %    \caption{CDF time reduction  CNN Cifar10}
    %    \label{fig:cost_cifar10}
    %\end{subfigure}


    \captionsetup{justification=justified}
    \caption{Standard and adversarial error correlation  between PGD20 and FGSM, PGD5, and PGD10 varying the bound $\epsilon$ %(Figures~\ref{fig:correlation_acc_imageNet_2} to \ref{fig:correlation_advacc_svhn_8}) 
    and CDF of the training time reduction obtained using cheaper AT algorithms w.r.t PGD20 (Figure~\ref{fig:cost_imageNet}). % to train a ResNet50 with ImageNet and a CNN with Cifar10.% Continuous and dashed lines correspond to standard and  adversarial error, respectively.
    }
     \label{fig:correlation}

\end{figure*}



\if0
\begin{figure*}[t]
\centering
    %\captionsetup{justification=justified, font=small}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[ trim=1mm 2mm 2.3cm 2.3cm, clip, width=\textwidth]{plots/imageNet/imageNet_epochs_correlation.pdf}
        \caption{Error Corr. ResNet50 ImageNet}
        %\caption{Error cor. ResNet}
        \label{fig:correlation_acc_imageNet}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[ trim=1mm 2mm 2.3cm 2.3cm, clip, width=\textwidth]{plots/imageNet/imageNet_epochs_correlation_AdvAcc.pdf}
        \caption{Adv. Error Corr. ResNet50 ImageNet}
        %\caption{Adv Error cor. ResNet}
        \label{fig:correlation_advacc_imageNet}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[ trim=1mm 2mm 2.3cm 2.3cm clip, width=\textwidth]{plots/svhn/svhn_epochs_correlation.pdf}
        \caption{Error Corr. ResNet18 SVHN} 
        %\caption{Error cor. CNN}
        \label{fig:correlation_acc_svhn}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[ trim=1mm 2mm 2.3cm 2.3cm clip, width=\textwidth]{plots/svhn/svhn_epochs_correlation_AdvAcc.pdf}
        \caption{Adv. Error Corr. ResNet18 SVHN}
        %\caption{Adv Error correlation CNN}
        \label{fig:correlation_advacc_svhn}
    \end{subfigure}

\vspace{2mm}
    
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[ trim=1mm 2mm 2.3cm 2.3cm clip, width=\textwidth]{plots/cifar10/cifar10_epochs_correlation.pdf}
        \caption{Error Corr. CNN Cifar10}
        %\caption{Error cor. CNN}
        \label{fig:correlation_acc_cifar10}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[ trim=1mm 2mm 2.3cm 2.3cm clip, width=\textwidth]{plots/cifar10/cifar10_epochs_correlation_AdvAcc.pdf}
        \caption{Adv. Error Corr. CNN Cifar10}
        %\caption{Adv Error correlation CNN}
        \label{fig:correlation_advacc_cifar10}
    \end{subfigure}
    \caption{Standard and adversarial error correlation between PGD using 20 iterations and FGSM for different bounds $\epsilon$ to train a ResNet50 with ImageNet and a CNN with Cifar10.
    }
     \label{fig:correlation2}
\end{figure*}



\fi

==> plots/heatmaps.tex <==
\begin{figure*}[t]
\centering
\captionsetup{justification=justified, font=small}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/imageNet/time/imageNet_time_ratios_heatmap_pgd_2.0_loss.pdf}
        \caption{Error ResNet50 ImageNet  $\epsilon$=2 }
        %\caption{Error PGD $\epsilon$=2}
        \label{fig:imageNet_time_acc_pgd_2}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=32cm 2mm 11cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/imageNet/time/imageNet_time_ratios_heatmap_pgd_2.0_loss.pdf}
        %\caption{Adv Err PGD $\epsilon$=2}
        \caption{Adv. Error ResNet50 ImageNet  $\epsilon$=2}
        \label{fig:imageNet_time_advacc_pgd_2}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/imageNet/time/imageNet_time_ratios_heatmap_pgd_4.0_loss.pdf}
        %\caption{Error PGD $\epsilon$=4}
        \caption{Error ResNet50 ImageNet $\epsilon$=4}
        \label{fig:imageNet_time_acc_pgd_4}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    %\centering
        \includegraphics[trim=32cm 2mm 6.5cm 2.5cm, clip, width=3cm,height=2.8cm]{plots/imageNet/time/imageNet_time_ratios_heatmap_pgd_4.0_loss.pdf}
        %\caption{Adv Err PGD $\epsilon$=4}
        \caption{Adv. Error ResNet50 ImageNet  $\epsilon$=4}
        \label{fig:imageNet_time_advacc_pgd_4}
    \end{subfigure}
    


   \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/svhn/time/svhn_time_ratios_heatmap_pgd_4.0_loss.pdf}
        \caption{Error ResNet18 SVHN  $\epsilon$=4}
        \label{fig:svhn_time_acc_pgd_4}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=32cm 2mm 11cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/svhn/time/svhn_time_ratios_heatmap_pgd_4.0_loss.pdf}
        \caption{Adv. Error ResNet18 SVHN  $\epsilon$=4}
        \label{fig:svhn_time_advacc_pgd_4}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/svhn/time/svhn_time_ratios_heatmap_pgd_8.0_loss.pdf}
        \caption{Error ResNet18 SVHN  $\epsilon$=8}
        \label{fig:svhn_time_acc_pgd_8}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=32cm 2mm 7cm 2.5cm, clip, width=3cm,height=2.8cm]{plots/svhn/time/svhn_time_ratios_heatmap_pgd_8.0_loss.pdf}
        \caption{Adv. Error ResNet18 SVHN  $\epsilon$=8}
        \label{fig:svhn_time_advacc_pgd_8}
    \end{subfigure}
\if0
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/svhn/time/svhn_time_ratios_heatmap_pgd_12.0_loss.pdf}
        \caption{Error $\epsilon$=12}
        \label{fig:svhn_time_acc_pgd_12}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=32cm 2mm 7cm 2.5cm, clip, width=3cm,height=2.8cm]{plots/svhn/time/svhn_time_ratios_heatmap_pgd_12.0_loss.pdf}
        \caption{Adv. Error $\epsilon$=12}
        \label{fig:svhn_time_advacc_pgd_12}
    \end{subfigure}
\fi

\if0
   \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_4.0_loss.pdf}
        %\caption{Error PGD $\epsilon$=4}
        \caption{Error $\epsilon$=4}
        \label{fig:cifar10_time_acc_pgd_4}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=32cm 2mm 11cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_4.0_loss.pdf}
        %\caption{Adv Err  PGD $\epsilon$=4}
        \caption{Adv. Error  $\epsilon$=4}
        \label{fig:cifar10_time_advacc_pgd_4}
    \end{subfigure}
\fi
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_8.0_loss.pdf}
        %\caption{Error PGD $\epsilon=8$}
         \caption{Error CNN Cifar10 $\epsilon=8$}
        \label{fig:cifar10_time_acc_pgd_8}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=32cm 2mm 11cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_8.0_loss.pdf}
        %\caption{Adv Err  PGD $\epsilon$=8}
        \caption{Adv. Error  CNN Cifar10  $\epsilon$=8}
        \label{fig:cifar10_time_advacc_pgd_8}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_12.0_loss.pdf}
        %\caption{Error PGD $\epsilon$=12}
        \caption{Error  CNN Cifar10 $\epsilon$=12}
        \label{fig:cifar10_time_acc_pgd_12}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[trim=32cm 2mm 7cm 2.5cm, clip, width=3cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_12.0_loss.pdf}
        %\caption{Adv Err  PGD $\epsilon$=12}
        \caption{Adv. Error   CNN Cifar10 $\epsilon$=12}
        \label{fig:cifar10_time_advacc_pgd_12}
    \end{subfigure}
\if0
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_16.0_loss.pdf}
        %\caption{Error PGD $\epsilon$=16}
        \caption{Error $\epsilon$=16}
        \label{fig:cifar10_time_acc_pgd_16}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[trim=32cm 2mm 7cm 2.5cm, clip, width=3cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_16.0_loss.pdf}
        %\caption{Adv Err PGD $\epsilon$=16}
        \caption{Adv. Error $\epsilon$=16}
        \label{fig:cifar10_time_advacc_pgd_16}
    \end{subfigure}
\fi

%\caption{Standard and adversarial test error training a CNN with Cifar10.}
\caption{Standard and adversarial test error training a ResNet50 ImageNet, ResNet18 SVHN, and CNN Cifar10 (stop condition time). PGD is used to generate adversarial examples, and the optimal configurations in the Pareto frontier are marked by a star.
}

\label{fig:heatmaps}


\end{figure*}









\if0

\begin{figure*}[t]
\centering
\captionsetup{justification=justified, font=small}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/imageNet/time/imageNet_time_ratios_heatmap_pgd_2.0_loss.pdf}
        \caption{Error $\epsilon$=2}
        %\caption{Error PGD $\epsilon$=2}
        \label{fig:imageNet_time_acc_pgd_2}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=32cm 2mm 11cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/imageNet/time/imageNet_time_ratios_heatmap_pgd_2.0_loss.pdf}
        %\caption{Adv Err PGD $\epsilon$=2}
        \caption{Adv. Error $\epsilon$=2}
        \label{fig:imageNet_time_advacc_pgd_2}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/imageNet/time/imageNet_time_ratios_heatmap_pgd_4.0_loss.pdf}
        %\caption{Error PGD $\epsilon$=4}
        \caption{Error $\epsilon$=4}
        \label{fig:imageNet_time_acc_pgd_4}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    %\centering
        \includegraphics[trim=32cm 2mm 6.5cm 2.5cm, clip, width=3cm,height=2.8cm]{plots/imageNet/time/imageNet_time_ratios_heatmap_pgd_4.0_loss.pdf}
        %\caption{Adv Err PGD $\epsilon$=4}
        \caption{Adv. Error $\epsilon$=4}
        \label{fig:imageNet_time_advacc_pgd_4}
    \end{subfigure}
    
\caption{Standard and adversarial test error training a ResNet50 with ImageNet (stop condition time). PGD is used to generate adversarial examples, and the optimal configurations in the Pareto frontier are marked by a star.
}
\label{fig:imageNet_time}

   \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/svhn/time/svhn_time_ratios_heatmap_pgd_4.0_loss.pdf}
        \caption{Error $\epsilon$=4}
        \label{fig:svhn_time_acc_pgd_4}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=32cm 2mm 11cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/svhn/time/svhn_time_ratios_heatmap_pgd_4.0_loss.pdf}
        \caption{Adv. Error $\epsilon$=4}
        \label{fig:svhn_time_advacc_pgd_4}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/svhn/time/svhn_time_ratios_heatmap_pgd_8.0_loss.pdf}
        \caption{Error $\epsilon$=8}
        \label{fig:svhn_time_acc_pgd_8}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=32cm 2mm 7cm 2.5cm, clip, width=3cm,height=2.8cm]{plots/svhn/time/svhn_time_ratios_heatmap_pgd_8.0_loss.pdf}
        \caption{Adv. Error $\epsilon$=8}
        \label{fig:svhn_time_advacc_pgd_8}
    \end{subfigure}
\if0
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/svhn/time/svhn_time_ratios_heatmap_pgd_12.0_loss.pdf}
        \caption{Error $\epsilon$=12}
        \label{fig:svhn_time_acc_pgd_12}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=32cm 2mm 7cm 2.5cm, clip, width=3cm,height=2.8cm]{plots/svhn/time/svhn_time_ratios_heatmap_pgd_12.0_loss.pdf}
        \caption{Adv. Error $\epsilon$=12}
        \label{fig:svhn_time_advacc_pgd_12}
    \end{subfigure}
\fi

\caption{Standard and adversarial test error training a ResNet18 with SVHN.}
\label{fig:svhn_time}




\if0
   \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_4.0_loss.pdf}
        %\caption{Error PGD $\epsilon$=4}
        \caption{Error $\epsilon$=4}
        \label{fig:cifar10_time_acc_pgd_4}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=32cm 2mm 11cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_4.0_loss.pdf}
        %\caption{Adv Err  PGD $\epsilon$=4}
        \caption{Adv. Error  $\epsilon$=4}
        \label{fig:cifar10_time_advacc_pgd_4}
    \end{subfigure}
\fi
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_8.0_loss.pdf}
        %\caption{Error PGD $\epsilon=8$}
         \caption{Error $\epsilon=8$}
        \label{fig:cifar10_time_acc_pgd_8}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=32cm 2mm 11cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_8.0_loss.pdf}
        %\caption{Adv Err  PGD $\epsilon$=8}
        \caption{Adv. Error  $\epsilon$=8}
        \label{fig:cifar10_time_advacc_pgd_8}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_12.0_loss.pdf}
        %\caption{Error PGD $\epsilon$=12}
        \caption{Error $\epsilon$=12}
        \label{fig:cifar10_time_acc_pgd_12}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[trim=32cm 2mm 7cm 2.5cm, clip, width=3cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_12.0_loss.pdf}
        %\caption{Adv Err  PGD $\epsilon$=12}
        \caption{Adv. Error  $\epsilon$=12}
        \label{fig:cifar10_time_advacc_pgd_12}
    \end{subfigure}
\if0
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[trim=5cm 2mm 38cm 2.5cm, clip, width=2.8cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_16.0_loss.pdf}
        %\caption{Error PGD $\epsilon$=16}
        \caption{Error $\epsilon$=16}
        \label{fig:cifar10_time_acc_pgd_16}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[trim=32cm 2mm 7cm 2.5cm, clip, width=3cm,height=2.8cm]{plots/cifar10/time/cifar10_time_ratios_heatmap_pgd_16.0_loss.pdf}
        %\caption{Adv Err PGD $\epsilon$=16}
        \caption{Adv. Error $\epsilon$=16}
        \label{fig:cifar10_time_advacc_pgd_16}
    \end{subfigure}
\fi

\caption{Standard and adversarial test error training a CNN with Cifar10.}
\label{fig:cifar10_time}


\end{figure*}

\fi

==> sections/1_abstract.tex <==
This work focuses on the problem of hyper-parameter tuning (HPT) for robust (i.e., adversarially trained) models, shedding light on the new challenges and opportunities 
arising during the HPT process for robust models.
%that emerge when performing HPT for robust models.
\if 0
%; ii) proposing novel
techniques to reduce these costs, by exploiting novel opportunities that emerge
in this conte

with the twofold goal of i)
establishing which additional HPs are relevant to tune in adversarial settings, and ii) reducing the cost of HPT for robust models.% by exploiting novel opportunities that emerge in this context.
\fi
To this end, we conduct an extensive experimental study based on three popular deep models and explore exhaustively nine (discretized)  hyper-parameters (HPs), two fidelity dimensions, and two attack bounds, for a total of 19208 configurations (corresponding to 50 thousand GPU hours).

Through this study, we show that the complexity of the HPT problem is further exacerbated in adversarial settings due to the need to independently tune the HPs used during standard and adversarial training: 
%failing to do so (i.e., adopting the same HP settings in both training phases) can  lead to an increase of up to 5$\times$ and 1.5$\times$ of the error for clean and adversarial inputs, respectively.
succeeding in doing so (i.e., adopting different HP settings in both  phases) can  lead to a reduction of up to 80\% and 43\% of the error for clean and adversarial inputs, respectively.
%
We also identify new opportunities to reduce the cost of HPT for robust models. 
Specifically, we propose to leverage cheap adversarial training methods to obtain inexpensive, yet highly correlated, estimations of the quality achievable using more robust/expensive state-of-the-art methods. We show that, by exploiting this novel idea in conjunction with a recent multi-fidelity optimizer (taKG), the efficiency of the HPT process can be enhanced by up to 2.1$\times$.

%In fact, besides introducing additional HPs,  due to two main reasons: i) the need of tuning additional HPs which balance standard and adversarial training; ii)  the need of tuning the HPs of these two training phases independently.
%Fortunately, we also identify new  opportunities to reduce the cost of HPT for robust models. 
%Specifically, we propose to leverage cheap adversarial training methods to obtain inexpensive, yet highly correlated, estimations of the quality achievable using state-of-the-art  methods (PGD). We show that, by exploiting this novel idea in conjunction with  a recent multi-fidelity optimizer (taKG), the efficiency of the HPT process can be significantly enhanced.

%not only due to the need of tuning additional HPs but also due to performing HPT twice, first for clean data and then for adversarial training.



%This work focuses on the problem of hyper-parameter tuning (HPT) for robust (i.e., adversarially trained) models. We start by shedding light via an empirical study on two fundamental questions that arise when designing HPT approaches for robust models, namely: i) should adversarial training be preceded by an initial clean data training phase and, if so, ii) should the 2 phases adopt the same hyper-parameters (HPs)? We show that the use of an initial clean data training phase typically speeds up model's convergence, but that the optimal ratio of computational resources to be allocated to each training phase varies significantly across models and datasets, which suggests that this should be treated as an additional HP. We also show that reusing the best HPs for clean data training during the adversarial training phase can lead to a significant reduction in the final model's quality.

%Overall, these findings show that the HPT problem, already notoriously expensive, is exacerbated in adversarial settings not only due to the need of tuning additional HPs but also due to performing HPT twice, first for clean data and then for adversarial training.
%





\if0
%Problem of HPT is notoriosuly expensive, especially for large model. In adversarial settings the problem is exacerbated due to two main factors: i) adv.training techniques are inherently more expensive, which accordingly amplifies the cost of HPT; ii) adv. training exposes additional hyper-parameters (e.g., ..), which further increases the search space.
%



We start by analyzing the impact of having an initial clean data training phase


Recent research has demonstrated that Machine Learning models are vulnerable to adversarial examples, i.e., perturbed inputs that are almost indistinguishable from clean data but cause models' misclassification.
To address this issue, adversarial training has emerged as a leading defense mechanism. %This approach generates and incorporates adversarial examples. 
Unfortunately, creating strong adversarial examples can be prohibitively expensive, making adversarial training techniques impractical on large and complex models and problems.



    
Therefore, in this work, we investigate the different trade-offs that arise during adversarial training, such as standard and adversarial accuracy, training and inference time, and the percentage of resources given to clean and adversarial training, in order to answer three main questions: 
i) Is it better to pre-train the model using only clean data or directly use adversarial training on a randomly initialized model?
ii) Assuming 2 phases for training (clean followed by adversarial training), should the same common hyper-parameters be used for both phases?
iii) Can the information on hyper-parameter tuning collected from cheap methods be used to inform expensive and more robust methods for adversarial training, given its high cost?



We conduct an extensive study that, to the best of our knowledge, is the first to explore the hyper-parameters optimization problem while performing adversarial training. We deployed different models using several benchmarks while varying the hyper-parameters and evaluated the quality of the models.
Our findings demonstrate that dividing the training of a robust model into 2 phases and independently tuning the respective hyper-parameters can yield significant improvements. Moreover, we show that cheap adversarial methods can be used to extrapolate the quality of better but expensive techniques while varying the hyper-parameters. 



Although adversarial training is one of the best defenses against adversarial attacks, its high cost hinders its adoption by the industry. Thus, our goal with this work is to reduce the cost and popularize adversarial training to ultimately increase the security and reliability of ML models.
\fi


==> sections/2_intro.tex <==
%\vspace{-3mm}
\section{Introduction}
\label{sec:2_intro}
%\vspace{-2mm}


% Adversarial training is important and inherently expensive: high level overview of the additional optimization problem in which you find smallest pertubation that maximizes loss and feed it back to the model. This is crucial for robustness but adds large additional costs.
%
% Another expensive, yet crucial phase in model building is HPT. In the context of adversarial models, the cost of HPT is exarcebated. Not only cost adv. training is more expensive than clean training, which makes more expensive to test individual configurations. But also there are additional hyper-parameters that are inherent to adv. training and that also require tuning, which amplify the search space.

% In this work, we investigate the challenges and opportunities that arise when designing tools for  HPT of adv. robust models.

%Stick with the abstract strucuture.
%


Adversarial attacks~\cite{adv_train} aim at causing model misclassifications by introducing small perturbations in the input. White-box methods like Project Gradient Descent (PGD)~\cite{pgd} have been shown to be extremely effective in synthesizing perturbations that are small enough to be noticeable by humans, while severely hindering the model's performance. Fortunately, models can be hardened against this type of attack via a so-called ``Adversarial Training'' (AT) process. During AT, which typically takes place after an initial standard training (ST) phase~\cite{delay_adv_train},  adversarial examples are synthesized and added (with their intended label) to the training set. %Over the last years, 
Recently, several  AT methods have been proposed~\cite{adv_train,pgd,trades} that explore different trade-offs between robustness and computational efficiency. %Yet, at the current date, 
Unfortunately, the most robust AT methods impose significant overhead (up to $7\times$ in the models tested in this work) with respect to standard training. % d (i.e., clean data training).
%
%Adversarial training emerged as one of the most effective defenses against those attacks. However
%
%Although adversarial methods are crucial to train robust models, it imposes large additional costs on the training process:
%However, adversarial training is inherently expensive: 
%an additional optimization problem needs to be solved to compute the smallest perturbation to yield a model's misclassification that is next added to the clean data and fed to the model.
%


These costs are further amplified when considering another crucial phase of model building, namely hyper-parameter tuning (HPT). In fact, HPT methods require training a model multiple times using different hyper-parameter (HP) configurations. Consequently, the overheads introduced by AT lead also to an increase in the cost of HPT. %Besides this, AT methods come with their own HPs. This amplifies the dimensionality of the HP space to be optimized,  further exacerbating the cost of HPT.
Further, AT and ST share common HPs, which raises the question of whether AT should simply employ the same HP settings used during ST, or if a new HPT process should be executed to select different HPs for the AT phase. In the latter case, the dimensionality of the HP space to be optimized grows significantly,  exacerbating the HPT cost.


%In fact, as recent literature~\cite{delay_adv_train,inter_ST_AT} have shown that it is typically beneficial to have 

%out the benefits of performing ST before AT.
%Therefore, given the need for using two distinct training phases (ST followed by AT) and since the two phases share HPs, a new 
%question is raised of whether the HP settings of the AT phase should simply be inherited from ST or should  be tuned independently, which implies a significant growth of the dimensionality of the HP space.
%Further, AT and ST share common HPs, which raises the question of whether AT should simply inherit the HPs used by ST or if a new HPT phase should be run to allow tuning differently its HPs. In the latter case, clearly, the cost of HPT is further amplified. 
%This work focuses on the problem of HPT for adversarially trained models with the twofold goal of i) shedding light on the new challenges (i.e., additional costs) that emerge when performing HPT for robust models; ii) proposing novel techniques to reduce these costs, by exploiting novel opportunities that emerge in this context.


%robust models by exploiting novel opportunities that emerge in this context.



%This amplifies the dimensionality of the HP space to be optimized,  further exacerbating the cost of HPT.

%Moreover, this cost is exacerbated if we keep in mind that to maximize the model's quality, we need to perform hyper-parameter tuning (HPT), which is another expensive, yet crucial phase in model building. 
%In the context of adversarial models, the cost of HPT is exarcebated. 
%Not only the cost of adversarial training is more expensive than clean training, which makes it more expensive to test individual configurations, but also there are additional hyper-parameters that are inherent to adversarial training  that also require tuning, which amplifies the search space and therefore the cost.
%Although training robust ML models gained significant attention from the scientific community, its adoption in production is limited due to the high cost involved~\cite{zico}. 



%% Hence, this work focuses on the problem of HPT for adversarially trained
%models, with the twofold goal of: i )quantifying the relevance of doing hpt for AT, assuming that during ST we had already done HPT. The benefits can be up to 40% higher clean data error.... ii) motivated by the relevance of HPT for AT, we show novel ways to reducing the cost of HPT for
%robust models by exploiting novel opportunities that emerge in this context.

%Describe datasets
%Preliminary step for the first: 1) show that one cannot get away by avoiding ST at all and doing AT upfront. If we do that, we have 

%

%Hence, this work focuses on the problem of HPT for adversarially trained models, with the twofold goal of: 1) establishing which additional HPs are relevant to tune when building robust models; 2) reducing the cost of HPT for robust models by exploiting novel opportunities that emerge in this context.




%Regarding the first goal, we start (Section~\ref{sec:5_2PhaseTraining}) by addressing the following key question: \textit{given an available computational budget (e.g., GPU hours), should AT be preceded by an initial ST phase? Or can higher efficiency  be attained by applying AT techniques upfront? }%The answer to this question has a direct impact on the HPT problem, given that the need for using two distinct training phases (ST followed by AT) raises in its turn the question of whether to use distinct hyper-parameters in each of these phases. 

Hence, this work focuses on the problem of HPT for adversarially trained models with the twofold goal of i) shedding light on the new challenges (i.e., additional costs) that emerge when performing HPT for robust models, and ii) proposing novel techniques to reduce these costs, by exploiting opportunities that emerge in this context.

We pursue the first goal via an extensive experimental study based on 3 popular models/datasets widely used to evaluate AT methods % (ResNet50~\cite{resnet} with ImageNet~\cite{imagenet}, ResNet18 with SVHN~\cite{svhn} and CNN with Cifar10~\cite{cifar10})
(ResNet50/ImageNet, ResNet18/SVHN, and CNN/Cifar10). In this study, we discretize and exhaustively explore the HP space composed of up to nine HPs, which we evaluated considering two ``fidelity dimension''~\cite{smac,mtbo} for the training process and two attack strengths. Overall, we test a total of 19208 configurations and we make this dataset publicly accessible in the hope that it will aid the design of future HPT methods specialized for AT.
%

Leveraging this data, we investigate 
%We start by using this dataset to shed light on 
a key design choice for the HPT process of robust models, namely the decision of whether to adopt the same vs. different HP settings during AT and ST (for the common HPs in the 2 phases). To this end, we focus on 3 key HPs of deep models: learning rate, momentum, and batch size. Our empirical study shows that allowing the use of different HP settings during ST and AT  can bring substantial benefits in terms of model quality, by reducing up to 80\% and 43\%  the standard and adversarial error, respectively.






\if 0
2xLR - 2 
BS - 2
Mom 2 
Alpha  2
RAT - 4 + 1
AE - 4

RAT = 30,50,70 
    => 4 * 4 * 4 * 2 * 3 * 4 = 1536
RAT = 0 
    => 2*2*2 => 8
RAT= 100
    => 2*2*2*2*4 =  64

--- HPs : 1536 + 8 + 64 = 1608

2 fidelity dimensions :
    - 4 * 5 = 20 fidelity configurations
\fi


%, where we consider not only the allocation of different ratios of computational resources to the ST/AT phases but also the possibility (as suggested in prior work~\cite{hp_robust_ibm}) to use batches containing different percentages of clean and adversarial examples during  AT.
%\textcolor{red}{We conduct an extensive study, where we discretize and exhaustively explore the search space composed of six HPs and two fidelities which yields a global search space encompassing 19208 configurations using different models, benchmarks, and attack amplitude for AT.}
%TODO? Brag about the breadth of the study of HPs explored..
%
%We  show that in most of the observed scenarios, the best models are achieved by allocating part of the computational budget to ST, and only then use AT. Further, the optimal ratio of adversarial examples used during AT varies depending on the model and the bound of adversarial perturbations. Both this parameter and the ratio of computational budget allocated to ST are, thus, key HPs whose proper tuning can have a significant impact on model quality.%  first ST and then AT. the training into 2 phases (ST followed by AT) and combining clean and adversarial examples  when  performing AT. Further, the computational resources allocated to ST/AT should be addressed as an additional HP to be tuned.
    %... THIS HAS TO BE MORE EXPANDED THAN IN THE ABSTRACT AND HAVE A SHORT QUANTITATIVE DESCRIPTION.
    %\item 
%The answer to the above question has a direct impact on the HPT problem, given that the need for using two distinct training phases (ST followed by AT) raises in its turn the question of whether to use distinct settings for the HPs in common to the two training phases, which implies a significant growth of the dimensionality of the HP space.
%Based on these findings    
% Given the advantages of using an initial ST phase followed by a final AT phase, should the same settings of the (common) HPs  be used for both phases? 
%In our study (Section~\ref{sec:6_HPO}), we quantify the effect of tuning three key HPs (learning rate, momentum, and batch size) by using the same or distinct settings for each training phase. %We discretize the HP space in order to gather exhaustive measurements. % and consider a global HP space of 320 and 2560 configurations for the case of using common and distinct HP settings, respectively. 
%Our study shows that independently optimizing the common HPs of the 2 phases can bring substantial benefits, i.e.,  reductions of up to 5$\times$ and 1.5$\times$ for error and adversarial error, respectively.

%We conclude that there is a reduction of the optimal standard and adversarial errors by up to 16\% and 7\%, respectively when independently optimizing the common HPs of the 2 phases. 
    %TODO: We show that the answer is... THIS HAS TO BE MORE EXPANDED THAN IN THE ABSTRACT AND HAVE A SHORT QUANTITATIVE DESCRIPTION.
%\end{itemize}


Further, our study demonstrates that while the cost and complexity of HPT are heightened in adversarial settings, it also reveals that, in the context of robust models,  unique opportunities can be exploited to effectively mitigate these costs.
%However, if on the one hand, our study shows that the cost and complexity of HPT are amplified in adversarial settings, on the other hand, also shows that, in the context of robust models, one can also exploit unique opportunities to reduce these costs. 
%(due to the need of tuning additional HPs but also due to the need of performing HPT twice, first for AT and then for AT. % clean data and then for adversarial training.
%
%Fortunately, we also show that, in the context of robust models, there exist unique opportunities to reduce the cost of HPT. 
Specifically, we show that it is possible to leverage cheap AT methods to obtain inexpensive, yet highly correlated, estimations of the quality achievable using more robust/expensive methods (PGD \cite{pgd}). Besides studying the trade-offs between cost reduction and HP quality correlation with different AT methods, we extend a recent multi-fidelity optimizer (taKG~\cite{takg}) to incorporate the choice of the AT method as an additional dimension to reduce the HPT cost. We evaluate the proposed method using our dataset and show that incorporating the choice of the AT method as an additional fidelity dimension in taKG leads up to  2.1$\times$ speed-ups, with gains that extend up to 3.7$\times$ w.r.t. popular HPT methods, as HyperBand~\cite{hyperband}.

%this novel idea in conjunction with  a recent multi-fidelity optimizer (taKG), we show that the cost of HPT process can be reduced by up to \textcolor{red}{2.1$\times$ compared to state-of-the-art solutions}.

\if 0
%For the second objective, we first address a new question that allows evaluating new opportunities to extend current multi-fidelity HP optimizers to train robust models, namely:


%\begin{itemize}
    %\item 
    $\bullet$ Can the cost of HPT be reduced by testing HP configurations using cheaper (but less robust) AT methods?
    The results show a strong correlation between the different AT methods that allow multi-fidelity optimizers to evaluate cheap configurations and extrapolate expensive and more robust algorithms for AT while reducing costs and improving the quality of the recommended models.
%\end{itemize}


%Thus, in this work, we will first revisit and review the literature on training robust ML models and HPO (Section~\ref{sec:3_related_word}), and then conduct a study to answer the questions enumerated above (Section~\ref{sec:study}).
\fi



\if0
\textbf{PAO: reviewed up to here}
Thus, in this work, we will first revisit and review the literature on training robust ML models, adversarial training, and hyper-parameter optimization (HPO) (Section~\ref{sec:3_related_word}), and %secondly explore the different trade-offs encountered when training a robust model (e.g., standard and adversarial accuracy, training and inference time, and the ratio of cleaned and perturbed inputs while training) to answer the following questions:\\
then we conduct a study to answer two crucial questions that emerge when training  and developing HPO techniques for robust models:\\
\textbf{1)}  Should adversarial training be performed using a pre-train model with clean data or a randomly initialized model (Section~\ref{sec:5_2PhaseTraining})? The results show that a two-phase training (standard follow by adversarial training) can have benefits in the quality of the final models.\\ 
\textbf{2)} Assuming two-phase training, should the same common
HPs be used for both phases? Here, we study the impact on the model's quality of selecting the HPs in both phases (Section~\ref{sec:6_HPO}), and the results show that there are always gains if the HPs of the
two phases are tuned independently.\\
\textbf{3)} Can the information on HP tuning collected from cheap methods be used to inform expensive and more robust methods for adversarial training, given its high cost? At last, we investigate the use of HPO techniques that exploit multi-fidelity evaluations to leverage the information on HP tuning collected from cheap methods to infer expensive and more robust ones for adversarial training, while accounting for the respective costs (Section~\ref{sec:7_multiBudgets}). The results highlight that \textbf{red}{blah...}





Machine Learning (ML) techniques are widely used across various applications, and they represent a vital component of many security and sensitive systems~\cite{distillation,robustness,security,paypal}. 
Recent works~\cite{adv_attack,adv_train} have exposed several security concerns when using Deep Neural Network models (DNN) that highlight the importance of developing new methods to cope with and obey security requirements. Although a vast spectrum of these works focus on DNN, a wider range of modeling techniques also present similar vulnerabilities~\cite{robustDT,robustDT1} against adversarial attacks.




Adversarial attacks~\cite{adv_attack,adv_train} aim at misclassifying a  model's prediction by introducing a small perturbation in the input. In such attacks, malicious perturbations are determined based on the model and added to the clean data. Then, those are fed into the model with the goal to mislead it.
Moreover, ML models are also vulnerable to targeted attacks~\cite{target,target2}, where the attacker’s goal is to target a certain class and yield a model's misclassification in one specific class.
Targeted attacks can be particularly dangerous in scenarios where misclassification of a specific class can cause significant harm or damage.




Many sensitive applications exploit ML techniques and must address these vulnerabilities and ensure that the model does not misclassify when the attacker introduces a small perturbation to the clean input. 
For example, autonomous driving cars leverage several AI and ML techniques (e.g., image recognition models) as a fundamental component of the interaction with the environment/world. Furthermore, a model’s misclassification can have catastrophic consequences and potentially leading to fatal accidents. Thus, these models should cope with possible adversarial examples that might surge in the real world. 
%For example, Eykholt et al.~\cite{stop} showed that the introduction of some stickers in a predefined position in a stop sign can mislead the model, and instead of being classified as a “stop sign”, the model will predict a speed limit sign.
%Another example of applications vulnerable to adversarial or target attacks arises from the credit card fraud detection industries where ML is a core component~\cite{feedzai,fraudDetection}. In this case, a misclassification can lead to large losses of capital and investments. These systems should be able to detect and cope with small changes in the input/feature space created by attackers and classify those as fraud.
Moreover, there are numerous examples of adversarial attacks across different domains as image recognition~\cite{adv_train}, text classification~\cite{adv_attack_text,adv_attack_text2}, malware detection~\cite{adv_attack_code}, and speech recognition~\cite{adv_attack_sound}.
This highlights the aggressiveness of adversarial attacks and underscores the need for developing robust ML models that can withstand those in different domains.
In recent years, several works~\cite{adv_train,pgd,distillation,zero_opt,deepfool} investigated and developed different techniques to mitigate these vulnerabilities by training robust models. Those works can be divided into four main areas: 
i) adversarial training~\cite{adv_train,pgd,fgsm_fast,fgsm_free}, 
ii) detection of adversarial attacks~\cite{detection,detection1,detection2}, 
iii) pre-processing techniques~\cite{preprocess,preprocess1,preprocess2}, 
and iv) verification and provable defenses~\cite{verification2,verification}.
Moreover, these different methods take different assumptions about the model (e.g, white or black box model), the attacker capabilities, and optimization algorithms~\cite{adv_train,pgd,zero_opt,deepfool,distillation}. 
Despite all these different approaches, adversarial training is still the one that yields better defenses against adversarial attacks~\cite{zico}, and thus, this survey will solely focus on these methods. %For example, the detection of adversarial attacks/examples is an extremely difficult task because the attacker can mislead two or more models in a single attack at the same time~\cite{detection2}.
 


 
\fi

==> sections/3_relatedWork.tex <==

%\vspace{-2mm}
\section{Background and Related Work} 
%\vspace{-1mm}
%\section{Adversarial Training}
\label{sec:3_related_word}

In this section, we first provide background information on AT techniques (Section~\ref{subsec:AT}) and then discuss related works in the area of HPT (Section~\ref{subsec:HPT}).



%\vspace{-2mm}
\subsection{Adversarial Training} %\vspace{-1mm}
\label{subsec:AT}

Adversarial attacks aim at % are based on the idea of 
introducing small perturbations to input data, often small enough to be hardly perceivable by humans, with the goal to lead the model to generate an erroneous output.
%There are numerous examples of adversarial attacks across different domains as image recognition~\cite{adv_train}, text classification~\cite{adv_attack_text,adv_attack_text2}, malware detection~\cite{adv_attack_code}, and speech recognition~\cite{adv_attack_sound}.
These attacks reveal vulnerabilities of current model training techniques, underscoring the need for developing robust models in different domains.
Thus, several works \cite{adv_train,pgd,fgsm_fast,fgsm_free,deepfool}  developed new techniques to mitigate these vulnerabilities and defend against adversarial attacks, by tackling them via different and often orthogonal or complementary ways, such as adversarial training~\cite{adv_train,pgd,fgsm_fast,fgsm_free},  detection of adversarial attacks~\cite{detection}, or
 pre-processing techniques to filter adversarial perturbations~\cite{preprocess}. 
Next, we will review existing AT approaches, which represent the focus of this work.


\if 0
Those works can be divided into four main areas: 
i) adversarial training~\cite{adv_train,pgd,fgsm_fast,fgsm_free}, 
ii) detection of adversarial attacks~\cite{detection,detection1,detection2}, 
iii) pre-processing techniques to automatically remove adversarial perturbations ~\cite{preprocess,preprocess1,preprocess2}, 
and iv) verification and provable defenses~\cite{verification2,verification}. 

These techniques tackle adversarial attacks in different, and often orthogonal or complementary ways. In the following, we will focus on reviewing existing approaches for AT, which are the ones more relevant for this work.
\fi

%Moreover, these different methods take different assumptions about the model (e.g, white or black box model), the attacker capabilities, and optimization algorithms~\cite{adv_train,pgd,zero_opt,deepfool,distillation}. 



%Despite all these different approaches, adversarial training is still the one that yields better defenses against adversarial attacks~\cite{zico}, and thus, this work will solely focus on these methods.
AT aims at improving the robustness of machine learning (ML) models by i) first generating adversarially perturbed inputs, and ii) feeding these adversarial examples, along with the correct corresponding label, during the model training phase. More formally, this process can be described as follows.
%lassic  training them on adversarial examples generated by injecting small perturbations into the original data. The perturbations are computed based on the current model and the clean inputs.
Unlike ST, which determines the models’ parameters $\theta$ by minimizing the loss function between the model's prediction for the clean input $f_{\theta }(x) $ and the original class $y$, i.e.,
$ \underset{\theta}{\min} \{  \underset{x,y \sim D}{\mathbf{E}} [L(f_{\theta}(x), y)] \}$, 
AT first computes a perturbation $\delta$, smaller than a maximum predefined bound $\epsilon$, which will mislead the current model, and then trains the model with that perturbed input. %adversarial input (the clean data input plus the perturbation).   
This approach leads to the  formulation of the following optimization problem: 
$\underset{\theta}{\min} \{ \underset{x,y \sim D}{\mathbf{E}} [ \underset{\|\delta \| < \epsilon}{\max} L(f_{\theta}(x+\delta), y) ] \}$.
%It should be noted that 
The model's robustness depends on the bound $\epsilon$ used to produce the adversarial examples and on the strength of the method used to compute those examples.







Several methods have been developed to solve this optimization problem (or variants thereof as, e.g., \cite{trades}) and the resulting techniques are based on different assumptions about, e.g., the availability of the model for the attacker (i.e., white-box~\cite{pgd} or black-box~\cite{black_box_adv_train}), whether the underlying model is differentiable~\cite{adv_train} or not~\cite{black_box_adv_train},  and the existence of bounds on attacker capabilities~\cite{deepfool}.
%
%Despite all these different approaches, adversarial training is still the one that yields better defenses against adversarial attacks~\cite{zico}, and thus, this work will solely focus on these methods. %For example, the detection of adversarial attacks/examples is an extremely difficult task because the attacker can mislead two or more models in a single attack at the same time~\cite{detection2}.
%There are three main strategies to train robust models that are related to lower bounds, exact solutions, and upper bounds.  
Among these techniques, two of the most popular ones are Fast Gradient Sign Method (FGSM)~\cite{adv_train} and Project Gradient Descent (PGD)~\cite{pgd}). Both techniques hypothesize that attackers can inject bounded perturbations and have access to a differentiable model. %Both methods solve first the inner maximization problem to find the perturbation and then the outer minimization problem to determine the models’ parameters. 
%However, these techniques require the computation of the gradient, which is not always possible. 
%
FGSM, and its later variants~\cite{fgsm_fast,fgsm_free,fgsm2}, rely on gradient descent to compute small perturbations in an efficient way. More in detail, for a given clean input $x$, this method adjusts the perturbation $\delta$ by the magnitude of the bound in the direction of the gradient of the loss function, i.e., $\delta = \epsilon \cdot \text{sign} (\nabla_{\delta} L (f_{\theta} (x+\delta), y ))$.
PGD iteratively generates adversarial examples by taking small steps in the direction of the gradient of the loss function and projecting the perturbed inputs back onto the $\epsilon$-ball around the original input, i.e., 
$\textit{Repeat:\hspace{3mm}} \delta = \mathcal{P} (\delta + \alpha \nabla_{\delta} L (f_{\theta} (x+\delta), y ) )$, where $\mathcal{P}$ is the projection onto the ball of radius $\epsilon$ and $\alpha$ can be seen as analogous to the learning rate in gradient-descent-based training. 
Due to its iterative nature, PGD incurs a notably higher computational cost than FGSM~\cite{fgsm_free,fgsm_fast}, but it is also regarded as one of the strongest methods to generate adversarial examples.
In fact, prior work has shown that PGD attacks can fool robust models trained via FGSM and that PGD-based AT produces models robust to larger perturbations~\cite{pgd}  and with higher adversarial accuracy.  
FGSM is also known to suffer from catastrophic-overfitting~\cite{catastrophic_overfitting}, in which the model's adversarial accuracy collapses after some training iterations.  
%
Henceforth, we will focus on FGSM and PGD, which, as mentioned, are among the most widely used and effective methods for generating adversarial examples~\cite{fgsm2}.  In fact, these methods have been extensively studied and compared in the literature~\cite{fgsm2,catastrophic_overfitting,fgsm_free,fgsm_fast} and represent a natural starting point for investigating the trade-offs related to HPT that arise in the context of AT.




\if0
\noindent \textbf{Fast Gradient Sign Method.}
%\vspace{2mm}
More in detail, in order to solve the inner optimization problem, we can rely on Gradient Descent (or Ascent) methods. Moreover, for a given clean input $x$, this method adjusts the perturbation $\delta$ in the direction of its gradient. The gradient $g = \nabla_{\delta} L (f_{\theta} (x+\delta), y )$
can be easily computed using backpropagation technique. The perturbation $\delta$ is then adjusted according to $\delta = \delta + \alpha g$,
for a given $\alpha$, and then projected into the norm ball defined by $\| \delta \| \leq \epsilon $. However, if we select a value of $\alpha$ big enough and consider the projection into the ball, the value of $g$ will not matter (only the sign of $g$, i.e., gradient direction) and the second term above equation can only take the values of $\pm \epsilon$. Thus, the perturbation can be easily obtained by computing $\delta = \epsilon \cdot \text{sign} (g)$.   %Equation~\ref{perturbation}.
%\begin{equation}
%	\delta = \epsilon \cdot \text{sign} (g)
%	\label{perturbation}
%\end{equation}
%
FGSM was one of the first methods to generate adversarial examples being proposed. However, the FGSM only allows the definition of $L_{\infty}$ norms, and it was proven that stronger methods can mislead models trained adversarially using FGSM~\cite{pgd,zico,fgsm_fast}.




\noindent \textbf{Projected Gradient Descent.}
The PGD method~\cite{pgd} does not make the assumption that $\alpha$ is large enough, and solves the inner maximization problem through the project gradient descent with a smaller step size and iteratively projects the result into the ball, i.e., 
$	\textit{Repeat:\hspace{3mm}} \delta = \mathcal{P} (\delta + \alpha \nabla_{\delta} L (f_{\theta} (x+\delta), y ) )$
%\begin{equation}
%	\text{Repeat:\hspace{3mm}} \delta = \mathcal{P} (\delta + \alpha \nabla_{\delta} L (f_{\theta} (x+\delta), y ) )
%	\label{pgd}
%\end{equation}
where $\mathcal{P}$ is the projection onto the ball of radius $\epsilon$. PGD allows more choices of the HPs (in particular, the step size $\alpha$ and number of iterations) and different norms (e.g., $L_1$, $L_2$, $L_{\infty}$ norms).
%
In spite of PGD presenting a significantly higher computational cost than FGSM, it is one of the strongest methods to generate adversarial examples.
Moreover, PGD attacks can mislead robust models trained via FGSM, yield models with higher adversarial accuracy, and allow the use of larger bounds~\cite{pgd}.  





There are several algorithms that extend both FGSM and PGD in order to improve their efficiency and performance. For example, Free At~\cite{fgsm_free} considers a mini-batch of samples where it computes the perturbations via FGSM but using a non-zero initialization (the value of the previous perturbation in the mini-batch is used to initialize the perturbation of a new sample). On the other hand, Fast AT~\cite{fgsm_fast} considers a non-zero random initialization of the perturbation. % and shows improvements in the adversarial accuracy of FGSM comparable to those achieved by PGD.
%


There are also other methods in the literature t


as, for example, DeepFool~\cite{deepfool} where the algorithm projects the clean input onto the closest decision hyperplane using a $L_{\infty}$ norm, or Zero-th Order Optimization~\cite{zero_opt} that considers a black-box approach and just queries the real model without calculating the gradients and adapts the perturbation accordingly with the output.
TRADES~\cite{trades} presents a new optimization problem that trades off adversarial robustness against accuracy.
It is also possible to solve a Mixed Integer Linear Programming optimization problem to determine small perturbations that mislead the model~\cite{robust_dts2}. However, this last method presents a significant additional cost to solve the optimization problem. 

\fi

%These vulnerabilities are encountered in different modeling techniques. For example, another class of attacks and defenses were developed particularly for robust decision trees, where the model is not differentiable. More in detail, Papernot et al.~\cite{robust_dts} present a method that reconstructs the path in the tree until a leaf node where the prediction is outputted, searches in the neighbor leaves to find a new path that will result in a different prediction, and change the input features accordingly to misclassify the model. 


%All these methods to train robust models have their own assumptions, trade-offs, pros, and cons. 
%In the rest of the work, 

%Moreover, adversarial training introduces new HPs to the optimization problem. Thus, to train robust models, we need not only to perform the standard training to determine the models’ parameters but also to compute the perturbations for the clean data. Thus, the difficulty of the problem increases considerably when compared with standard training with clean data. 


Independently of the technique used to perform AT, a relevant finding, first investigated by \cite{delay_adv_train}, %Gupta et al.~\cite{delay_adv_train}, 
is whether to use an initial ST phase before performing AT, or whether to use exclusively AT.  %This study has shown that the use of an initial ST phase normally helps improving model's quality, especially when a limited computational budget (e.g., GPU time or epochs) is available for training. 
This study showed that using an initial ST phase normally helps to reduce the computational cost while yielding models with comparable quality. 
This result motivates one of the key questions that we aim at answering in this work, namely whether the ST and AT phases should share the settings for their common HPs. %Note that we have verified that the use of an initial ST phase is beneficial also for our models/datasets, even when considering an additional alternative, namely using batches that contain both clean and adversarial data (see Fig.~\ref{xxxx}).



%(which we verified to hold  also for our models/datasets, see Fig.~\ref{xxxx}) is 

%Our work is also related to the study by Gupta et al.~\cite{delay_adv_train}, which evaluated the impact of having the AT phase preceded by an initial ST. This study has shown that the use of an initial ST phase normally helps improving model's quality, especially when a limited computational budget (e.g., GPU time or epochs) is available for training. Motivated by this result (which we verified to hold  also for our models/datasets, see Fig.~\ref{xxxx}), we investigate


%However, our study considers a broader number of factors and in particular the possibility to use batches that contain both clean and adversarial data when doing AT. 
%Our results show that there exist several settings %(e.g., Figures \ref{fig:svhn_time_acc_pgd_4},  \ref{fig:svhn_time_advacc_pgd_4}, 
%\ref{fig:svhn_time_acc_pgd_12},  \ref{fig:svhn_time_advacc_pgd_12}, 
%\ref{fig:cifar10_time_acc_pgd_4}, and \ref{fig:cifar10_time_advacc_pgd_4}) 
%in which constraining the training to use batches composed exclusively of clean or adversarial examples leads to suboptimal models. 
%Based on our study, we advocate that both these ratios should be treated as hyper-parameters to be tuned depending on the application's needs. Further, we propose novel and efficient ways to explore the HP space in AT settings, namely  taking advantage of cheap adversarial methods to assess the quality of given HP settings.


\subsection{Hyper-parameter Tuning} 
\label{subsec:HPT}



HPT is a critical phase to optimize the performance of ML models. As the scale and complexity of models increase, along with the number of HP that can possibly be tuned in modern ML methods~\cite{nlp-paper-tuning}, %~\cite{klein2020model,nas_hpt}
HPT is a notoriously  time-consuming process, whose cost can become prohibitive due to the need to repetitively train complex models on large datasets. 




%o address this issue, state-of-the-art solutions exploit cheap low-fidelity models (e.g., trained with a fraction of the available data) to extrapolate the quality of fully trained models. This approach saves time and resources while still providing accurate estimates for different configurations.





To address this issue, a large spectrum of the literature on HPT relies on Bayesian Optimization (BO) %\cite{trimtuner,fabolas,ei,mtbo,takg,lynceus,cherrypick,smac,freeze-thawBO,loss_NN_gps,bo_stop,Vizier,mes-par,ucb-mf-gp,mf-hp,miso,general-mfbo,kg}
\cite{trimtuner,fabolas,ei,mtbo,takg,lynceus,smac,freeze-thawBO}. BO employs modeling techniques (e.g., Gaussian Processes) to guide the optimization process and leverages the model's knowledge and uncertainty (via a, so called, acquisition function) to select which configurations to test.
%~\cite{gps}, Random Forest~\cite{Random_Forest}, or Tree Parzen  to select the most promising HPs  to explore. 
%BO employs a model of the objective function to be optimized relying on modeling techniques such as Gaussian Processes, %~\cite{gps}, Random Forest~\cite{Random_Forest}, or Tree Parzen Estimators (TPE)~\cite{tpe} 
%, striving to identify promising configurations.% and increasing convergence speed. 
Although the use of BO can help to increase the convergence speed of the optimization process, the cost of testing  multiple HP configurations can quickly become prohibitive, especially when considering complex models trained over large datasets.
%can quickly become 

%-sets is often prohibitiv ewhen larger search spaces are considered, the convergence of BO methods is very slow~\cite{trimtuner}. 

To tackle this problem, multi-fidelity techniques~\cite{smac,mtbo,fabolas,trimtuner,freeze-thawBO,takg}  exploit cheap low-fidelity evaluations (e.g., training with a fraction of the available data or using a reduced number of training epochs) and extrapolate this knowledge to recommend high-fidelity configurations. This allows for reducing the cost of testing HP configurations, while still providing useful information to guide the search for the optimal high-fidelity configuration(s)~\cite{smac,trimtuner}. 
%
%
%Conversely, 
HyperBand~\cite{hyperband} is a popular multi-fidelity and model-free approach that promotes good quality configurations to higher budgets and discards the poor quality ones using a simple, yet effective, successive halving approach~\cite{successiveHalving}. Several approaches extended HyperBand using models to identify good configurations \cite{bohb,dehb} or shortcut the number of configurations to test~\cite{hyperjump}.
While these works adopt a single budget type (e.g., training time or dataset size), other approaches, such as taKG~\cite{takg}, make joint usage of multiple budget/fidelity dimensions during the optimization process to have additional flexibility to reduce the optimization cost. taKG selects the next configuration and different budgets via model-based predictive techniques that estimate the cost incurred and information gained by sampling a given configuration for a given setting of the available fidelity dimensions.




%To the best of our knowledge, the problem of HPT for adversarially robust models has not been deeply investigated in the literature. % have been barely investigated in the context of adversarially   robust models. 
%Previous works that develo at training robust models~\cite{adv_train,pgd,fgsm_fast,fgsm_free,fgsm2} fixed the HPs to train the model, which might yield lower quality models. The best HP choices for ST are likely to be no longer optimal for AT.
%Duesterwald et al.~\cite{hp_robust_ibm} studied the impact on the standard and adversarial accuracy when training an ML model of increasing the perturbation magnitude and percentage of adversarial inputs. Moreover, they proposed an optimization problem to maximize robustness constrained to a maximum reduction in the standard accuracy. In this approach, they resort to grid-search, random search, and BO with Tree-structured Parzen Estimator~\cite{tpe} to just tune these two previous parameters (while fixing the training HP).
%On the other hand, Gupta et al.~\cite{delay_adv_train} show that the quality of a model can be maintained when delaying adversarial training and  initial training with natural samples. 
%
%%%


In the area of HPT for robust models, the work that is more closely related to ours is the study by \cite{hp_robust_ibm}. %Duesterwald et al.~\cite{hp_robust_ibm}. 
This work has investigated empirically the relations between the bounds on adversarial perturbations ($\epsilon$) and the model's accuracy/robustness. Further, it showed that the ratio of clean/adversarial examples included in a batch (during AT) can have a positive impact on the model's quality and represents, as such, a key HP. Based on this finding, we incorporate this HP among the ones tested in our study. %They also studied the impact of their tuning process on both clean and adversarial accuracy and proposed optimizing those using classical HPT techniques. 
Differently from that work, we focus on 
i) quantifying the benefits of using different HPs during ST and AT, 
%(\cite{hp_robust_ibm}  % \cite{hp_robust_ibm} %Duesterwald et al.~\cite{hp_robust_ibm} 
%considered only 2 HPs of the AT phase,
%considered a single, and common, setting for the HPs that affect both ST and AT, %ii) investigating the impact of using an initial ST phase, 
and ii) exploiting the correlation between cheaper AT methods (such as FGSM) to enhance the efficiency of multi-fidelity HPT algorithms.
%%
%
%
\if 0
Our work is also related to the study by Gupta et al.~\cite{delay_adv_train}, which evaluated the impact of having the AT phase preceded by an initial ST. This study has shown that the use of an initial ST phase normally helps improving model's quality, especially when a limited computational budget (e.g., GPU time or epochs) is available for training. Motivated by this result (which we verified to hold  also for our models/datasets, see Fig.~\ref{xxxx}), we investigate


However, our study considers a broader number of factors and in particular the possibility to use batches that contain both clean and adversarial data when doing AT. 
%Our results show that there exist several settings %(e.g., Figures \ref{fig:svhn_time_acc_pgd_4},  \ref{fig:svhn_time_advacc_pgd_4}, 
%\ref{fig:svhn_time_acc_pgd_12},  \ref{fig:svhn_time_advacc_pgd_12}, 
%\ref{fig:cifar10_time_acc_pgd_4}, and \ref{fig:cifar10_time_advacc_pgd_4}) 
%in which constraining the training to use batches composed exclusively of clean or adversarial examples leads to suboptimal models. 
Based on our study, we advocate that both these ratios should be treated as hyper-parameters to be tuned depending on the application's needs. Further, we propose novel and efficient ways to explore the HP space in AT settings, namely  taking advantage of cheap adversarial methods to assess the quality of given HP settings.
}


\fi 

==> sections/4.2_tables.tex <==

\begin{table}[t]
\centering
    \begin{tabular}{c|c} 
    \textbf{Hyper-parameter} & \textbf{Values} \\\hline \hline
    %
    Learning Rate (ST and AT)  &  \{0.1, 0.01\}  \\\hline 
    %
    \multirow{2}{*}{Batch Momentum (ST and AT)}   & \{0.9, 0.99\} for ResNet50  \\
    &  \{0, 0.9\} otherwise\\\hline 
    %
    \multirow{2}{*}{Batch Size (ST and AT)}  & \{256, 512\} for ResNet50 \\
    &  \{128, 256\} otherwise\\\hline

     $\alpha$ (PGD learning rate)& \{$10^{-2}$, $10^{-3}$\} \\ \hline 
     %
     %No. of Iterations & \{5, 10, 20\} \\ \hline
     %
     % Percentage of adversarial resources
     %\% resources (time or epochs) for AT (\%RAT) & \{0, 30, 50, 70, 100\} \\     \hline
     \% resources (time or epochs) & \multirow{2}{*}{ \{0, 30, 50, 70, 100\}} \\
    for AT (\%RAT) &  \\\hline
      %
     %Percentage of adversarial examples
     %\% adversarial examples in each batch (\%AE) &  \{30, 50, 70, 100\} \\%[2mm]
    \% adversarial examples  & \multirow{2}{*}{ \{30, 50, 70, 100\} }\\%[2mm]
    in each batch (\%AE) &
     \end{tabular}
    \caption{Hyper-parameters considered}
    \label{tab:fixed_hp}
    \vspace{4mm}
%\end{table}

%\begin{table}[t]
\centering
    \begin{tabular}{ c|c } 
        \textbf{Model \& Benchmark} & \textbf{Bound $\epsilon$} \\\hline \hline
        ResNet50/ImageNet & \{2, 4\} \\ \hline
        ResNet18/SVHN & \{4, 8\} \\ \hline
        CNN/Cifar10 & \{8, 12\} \\%[2mm]
    \end{tabular}
    \caption{Bounds $\epsilon$ per benchmarks}
    \label{tab:bounds}
    \vspace{4mm}
%\end{table}

%\begin{table}[t]
\centering
    \begin{tabular}{ c|c } 
        \textbf{Fidelities}  &\textbf{Values} \\\hline \hline
        PGD iterations &  \{1 (FGSM), 5, 10, 20\} \\ \hline
        Epochs & \{1,2,4,8,16\} \\%[2mm]
        \end{tabular}
        \caption{Fidelities considered}
    \label{tab:budgets}
\end{table}





\if0
\begin{table*}[t]
    \begin{minipage}{.6\linewidth}

 %   \centering
    \begin{tabular}{c|c} 
    \textbf{Hyper-parameter} & \textbf{Values} \\\hline \hline
    %
    Learning Rate (ST and AT)  &  \{0.1, 0.01\}  \\\hline 
    %
    \multirow{2}{*}{Batch Momentum (ST and AT)}   & \{0.9, 0.99\} for ResNet50  \\
    &  \{0, 0.9\} otherwise\\\hline 
    %
    \multirow{2}{*}{Batch Size (ST and AT)}  & \{256, 512\} for ResNet50 \\
    &  \{128, 256\} otherwise\\\hline

     $\alpha$ (PGD learning rate)& \{$10^{-2}$, $10^{-3}$\} \\ \hline 
     %
     %No. of Iterations & \{5, 10, 20\} \\ \hline
     %
     % Percentage of adversarial resources
     %\% resources (time or epochs) for AT (\%RAT) & \{0, 30, 50, 70, 100\} \\     \hline
     \% resources (time or epochs) & \multirow{2}{*}{ \{0, 30, 50, 70, 100\}} \\
    for AT (\%RAT) &  \\\hline
      %
     %Percentage of adversarial examples
     %\% adversarial examples in each batch (\%AE) &  \{30, 50, 70, 100\} \\%[2mm]
    \% adversarial examples  & \multirow{2}{*}{ \{30, 50, 70, 100\} }\\%[2mm]
    in each batch (\%AE) &
     \end{tabular}
     \vspace{-2mm}
    \caption{Hyper-parameters considered}
    \label{tab:fixed_hp}
%\vspace{-2mm}
\end{minipage}%
%
\begin{minipage}{.4\linewidth}
        \begin{tabular}{ c|c } 
            \textbf{Model \& Benchmark} & \textbf{Bound $\epsilon$} \\\hline \hline
            ResNet50/ImageNet & \{2, 4\} \\ \hline
            ResNet18/SVHN & \{4, 8\} \\ \hline
            CNN/Cifar10 & \{8, 12\} \\%[2mm]
        \end{tabular}
        \vspace{-2mm}
        \caption{Bounds $\epsilon$ per benchmarks}
        \label{tab:bounds}

        \vspace{2.0mm}
        \begin{tabular}{ c|c } 
        \textbf{Fidelities}  &\textbf{Values} \\\hline \hline
        PGD iterations &  \{1 (FGSM), 5, 10, 20\} \\ \hline
        Epochs & \{1,2,4,8,16\} \\%[2mm]
        \end{tabular}
        \vspace{-2mm}
        \caption{Fidelities considered}
        \label{tab:budgets}
    \end{minipage} 
%\vspace{-6mm}
\end{table*}







\begin{table*}[t]

\centering
\begin{tabular}{c|c} 
    \textbf{Hyper-parameter} & \textbf{Values} \\\hline \hline
    %
    Learning Rate (ST and AT)  &  \{0.1, 0.01\}  \\\hline 
    %
    \multirow{2}{*}{Batch Momentum (ST and AT)}   & \{0.9, 0.99\} for ResNet50  \\
    &  \{0, 0.9\} otherwise\\\hline 
    %
    \multirow{2}{*}{Batch Size (ST and AT)}  & \{256, 512\} for ResNet50 \\
    &  \{128, 256\} otherwise\\\hline

     $\alpha$ (PGD learning rate)& \{$10^{-2}$, $10^{-3}$\} \\ \hline 
     %
     %No. of Iterations & \{5, 10, 20\} \\ \hline
     %
     % Percentage of adversarial resources
     \% resources (time or epochs) for AT (\%RAT) & \{0, 30, 50, 70, 100\} \\ 
      \hline
      %
     %Percentage of adversarial examples
     \% adversarial examples in each batch (\%AE) &  \{30, 50, 70, 100\} \\%[2mm]
     \end{tabular}
     \vspace{-3mm}
\caption{Hyper-parameters considered}
\label{tab:fixed_hp}
%\vspace{-2mm}
    \begin{minipage}{.5\linewidth}
        \begin{tabular}{ c|c } 
            \textbf{Model \& Benchmark} & \textbf{Bound $\epsilon$} \\\hline \hline
            ResNet50 ImageNet & \{2, 4\} \\ \hline
            ResNet18 SVHN & \{4, 8\} \\ \hline
            CNN Cifar10 & \{8, 12\} \\%[2mm]
        \end{tabular}
        \vspace{-3mm}
        \caption{Bounds $\epsilon$ per benchmarks}
        \label{tab:bounds}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
        \begin{tabular}{ c|c } 
        \textbf{Fidelities}  &\textbf{Values} \\\hline \hline
        PGD iterations &  \{1 (FGSM), 5, 10, 20\} \\ \hline
        Epochs & \{1,2,4,8,16\} \\%[2mm]
        \end{tabular}
        %\vspace{4.0mm}
        \vspace{-2mm}
        \caption{Fidelities considered}
        \label{tab:budgets}
    \end{minipage} 
%\vspace{-6mm}
\end{table*}
\fi


==> sections/4_experimentsSetup.tex <==




%\vspace{-3mm}
\section{HPT for Robust Models: Challenges and Opportunities} 
%\vspace{-2mm}
\label{sec:study}

As mentioned, this work aims at shedding light on the challenges and opportunities that arise when performing HPT for adversarially robust models.
%
%As for the challenges, our focus is on clarifying the impact that adversarial training methods have on the complexity of the HPT problem. 
More precisely, we seek to answer the following questions:
\begin{enumerate}
%  \noindent \textbf{1)} 
  \item Should the HPs that are common to the AT and ST phases be tuned independently? More in detail, we aim at quantifying to what extent the model's quality is affected if one uses the same vs different HP settings during the ST and AT phases %We also show that the above question can not be  simply circumvented by avoiding to perform an initial ST phase and using exclusively AT. 
  (see Section~\ref{sec:6_HPO}).\\

  %\noindent \textbf{2)} 
  \item Is it possible to reduce the cost of HPT by testing HP settings using cheaper (but less robust) AT methods? How correlated are the performance of alternative AT approaches and what factors (e.g., the perturbation bound or the cost of the techniques) impact such correlation? To what extent can this approach enhance the HPT's process efficiency?  (see Section~\ref{sec:7_multiBudgets}.)
\end{enumerate}
%As for the opportunities that adversarial training enable for the design of HPT mechanisms, we investigate a novel idea: given the existence in the literature of alternat, 

In order to answer the above questions, we have collected (and made publicly available) a dataset, which we obtained by varying some of the most impactful HPs for three popular neural models/datasets and measured the resulting model quality. We provide a detailed description of the dataset in Section~\ref{sec:experiment}.


 

\input{4.2_tables}


%\vspace{-2mm}
\subsection{Experimental Setup}
\label{sec:experiment}
%\vspace{-1mm}

We base our study on 3 widely-used models and datasets (ResNet50/ImageNet, ResNet18/SVHN, and  CNN/Cifar10). 
All the models were trained using 1 worker, except SVHN which  2 workers were used.
We used Nvidia Tesla V100 GPUs to train the ResNet50, and  Nvidia  GeForce RTX 2080 for the remaining models. All models and training procedures were implemented in Python3 via the Pytorch framework.

To evaluate the models, we considered up to 9 different HPs, as summarized in Table~\ref{tab:fixed_hp}. The first 3 HPs in this table apply to both the ST and AT phases.  $\alpha$ is an HP that applies exclusively to AT, whereas the last 2 HPs (\%RAT and \%AE) regulate the balance between ST and AT (see Section~\ref{sec:3_related_word}). Specifically, \%RAT defines the number of computational resources allocated to the AT phase, and \%AE indicates the ratio of adversarial inputs contained in the batches during the AT phase (as suggested by \cite{hp_robust_ibm}). %Duesterwald et al.~\cite{hp_robust_ibm}).
%
We further consider several settings of the bound $\epsilon$ on the attacker power (see Table~\ref{tab:bounds}).
%Note that the reported values of $\epsilon$ are normalized by 255. 
Finally, we also consider two fidelity dimensions, namely the number of training epochs and the number of PGD iterations (see Section~\ref{sec:7_multiBudgets}). The model's quality is evaluated using standard error (i.e., error using clean inputs) and adversarial error (i.e., error using adversarially perturbed inputs).


For each model, we exhaustively explored the (discretized) space defined by the HPs, bound $\epsilon$, and fidelities, which yields a search space encompassing a total of 19208 configurations. Building this dataset required around 50 thousand GPU hours and we have made it publicly accessible in the hope that it will aid the design of future HPT methods specialized for AT. Additional information to ensure the reproducibility of results is provided in the public repository\footnote{\url{http://anonymous.4open.science/r/HPT_advTrain1}}.
%\footnote{\textcolor{red}{\url{https://github.com/pedrogbmendes/HPT\_advTrain}}}. %, and MNIST. 

%Overall, our dataset, which reports the models' error and adversarial for all the considered HPs, bounds and fidelities contain a  




%based on 3 different deep neural models and three datasets.





\if0
\begin{table*}[t]
\centering
\begin{tabular}{ c|c|c } 
    \textbf{Hyper-parameter} &  \textbf{Algorithm} & \textbf{Values} \\\hline \hline
    %
    Learning Rate  & STD, FGSM, PGD &  \{0.1, 0.01\}  \\\hline 
    \multirow{2}{*}{Momentum} & \multirow{2}{*}{STD, FGSM, PGD }  & \{0.9, 0.99\} for ResNet50  \\
     & &  \{0, 0.9\} otherwise\\\hline 
    % Momentum &  STD, FGSM, PGD  &  \{0.9, 0.99\} for ImageNet, \{0, 0.9\} otherwise\\\hline 
     %
     \multirow{2}{*}{Batch Size}  & \multirow{2}{*}{STD, FGSM, PGD } & \{256, 512\} for ResNet50 \\
     & &   \{128, 256\} otherwise\\\hline
     %Batch Size & STD, FGSM, PGD & \{256, 512\} for ImageNet,  \{128, 256\} otherwise\\\hline
     %
    \multirow{3}{*}{Bound $\epsilon$} & \multirow{3}{*}{FGSM, PGD }& \{2, 4\} for ResNet50 \\ 
     & &  \{4, 8, 12\} for ResNet18  \\ 
     & &  \{4, 8, 12, 16\} for CNN  \\ 
    % & & \{0.05, 0.1, 0.2, 0.3, 0.4, 0.5\} for MNIST \\ 
    \hline 
    %\multirow{3}{*}{Bound $\epsilon$} & \multirow{3}{*}{FGSM, PGD }& \{2, 4\} for ImageNet, \{4, 8, 12\} for SVHN,  \\ 
     %& &  \{4, 8, 12, 16\} for Cifar10,  \\ 
     %& & \{0.05, 0.1, 0.2, 0.3, 0.4, 0.5\} for MNIST \\ \hline 
     %
     $\alpha$ & PGD & \{$10^{-2}$, $10^{-3}$\} \\ \hline 
     %
     No. of Iterations & PGD & \{5, 10, 20\} \\ \hline
     %
      Percentage of adversarial resources & \multirow{2}{*}{FGSM, PGD} & \multirow{2}{*}{\{0, 30, 50, 70,100\}} \\ 
       for training (time or epochs) & & \\ 
      \hline
      %
     Percentage of adversarial  & \multirow{2}{*}{FGSM, PGD} &  \multirow{2}{*}{\{30, 50, 70,100\} }\\
     examples & & 
\end{tabular}

\caption{Hyper-parameters considered}
\label{tab:fixed_hp}


\end{table*}



\begin{table*}[t]
\centering
\begin{tabular}{ c|c } 
\textbf{Fidelities}  &\textbf{Values} \\\hline \hline
No. of Iterations &  \{FGSM, PGD5, PGD10, PGD20\} \\ \hline
Epochs & \{ 1,2,4,8,16  \}
\end{tabular}
\caption{Fidelities (budgets) considered}
\label{tab:fixed_hp}
\end{table*}
\fi

%\textcolor{red}{I think we should add a section here to explained the experiments (networks, benchmarks, hyper-paramters, etc considered in this study)}



\if 0
We used two stop conditions independently during training. 
First, we trained the ResNet50 using ImageNet and ResNet18 using SVHN  for 12 and 6 hours, respectively, while the CNN using Cifar10 was trained for 10 minutes. 
Next, we trained each model from scratch using the number of epochs as the stop condition (set to 16 epochs).
For a fair comparison, using the correct stop conditions is important depending on the research question that we aim to answer.
These datasets were collected over several months corresponding to more than 50 thousand GPU hours of computation.% and an investment of more than US\$26000.
We resort to Nvidia Tesla V100 GPUs to train the ResNet50 model, and to Nvidia  GeForce RTX 2080 for the remaining models. 
All models and training procedures were implemented in Python3 via the Pytorch framework.
\fi
%
%Due to space constraints, in the main body of the paper, we only report the result of ResNet50 using ImageNet and a CNN using Cifar10. Additional results are detailed in the supplemental material. 


%In the following sections, we answer the questions enumerated above.


==> sections/5_2PhaseTraining.tex <==


%\section{Clean vs. adversarial training}
\subsection{Should adversarial models be pre-trained with clean data?}
%Do adversarial benefit from an initial clean data training ?
\label{sec:5_2PhaseTraining}

\input{plots/heatmaps}

%\textbf{Should use a pre-train model using clean data only or directly use adversarial training on a randomly initialized model?}

%\subsection{ImageNet (stop condition time)}
%\input{plots/imageNet_time}

%\subsection{SVHN (stop condition time)}
%\input{plots/svhn_time}

%\subsection{CIFAR10 (stop condition time)}
%\input{plots/cifar10_time}

%\subsection{MNIST (stop condition time)}
%\input{plots/mnist_time}

In this section, we study two different approaches to train robust models: 1) using AT since the beginning of the training process, or 2) pre-train a model first using clean inputs and then using AT. % and then fine-tuning it using adversarial examples generated through the initialized model.
%
%When training a robust model, one can decide to train the model using adversarial examples from the beginning of the training process or train first using clean data and then "fine-tune" the model using adversarial examples generated through the initialized model. 
%
We further consider the option, first suggested by \cite{hp_robust_ibm}, %Duesterwald et al.~\cite{hp_robust_ibm},
%instead of pre-training a model with clean data, alternatively, one can also start training a model adversarially from scratch 
of mixing clean and adversarial data during AT to improve model convergence.
%during adversarial training, one can mix clean and adversarial data to improve the convergence of the model.

In order to compare these options, we train a robust model using PGD given the same global budget (e.g., training time or cloud cost), varying the strength of the adversarial attack (i.e., the adversarial bound), the percentage of AT time (\%RAT), and the percentage of adversarial examples while adversarially training the model (\%AE) and fixing the remaining hyper-parameters (using default values typically adopted in the literature for the considered models~\cite{fgsm2}).




Figure~\ref{fig:heatmaps} % \ref{fig:imageNet_time}, \ref{fig:svhn_time} and \ref{fig:cifar10_time} 
plots the standard and adversarial error varying the percentage of  AT time (\%RAT) and the percentage of adversarial examples while training adversarially (\%AE) using ResNet50/ImageNet, ResNet18/SVHN and a CNN/Cifar10, respectively.  
%We include plots  referring to other values of $\epsilon$ in the supplemental material.
%
For a fair comparison, we set the same global budget for each parameter's setting. In particular, ResNet50 was trained for 12 hours, ResNet18 was trained for 6 hours using 2 workers, and CNN was trained for 10 minutes.
Moreover, for each plot, we identify the optimal configurations that composed the Pareto frontier with a star. In particular, configurations that avoid the initial ST (i.e., \%RAT=100) correspond to the last row of the heatmaps.



% and the configurations close to the Pareto frontier (marked by a black star).




By analyzing the distribution of the Pareto optimal configurations, %(and accounting also for the scenarios included in the supplemental material), 
we observe that 60\% of the configurations in the Pareto frontiers performed some initial ST before training adversarially. In fact, only in one scenario out of nine different settings that we consider (i.e., 11\% of all the  scenarios (ResNet18 SVHN $\epsilon$=4, Fig.~\ref{fig:svhn_time_acc_pgd_4} and \ref{fig:svhn_time_advacc_pgd_4}), we see that ST can indeed be avoided, by resorting to a mix of clean and adversarial examples during AT. It should be noted that this scenario corresponds to the lowest settings of the bound for that model/benchmark, and when using larger bounds $\epsilon$ also with this model/dataset we observe a growing ratio of Pareto frontier configurations that use both ST and AT.

We argue that these results can be explained by considering that the examples generated during AT depend on the current state of the model. As such,  by generating upfront adversarial examples using a random initialized (i.e., not pre-trained with clean data) model, one incurs the risk of misspending computational resources by synthesizing non-effective/random perturbations. Further, when larger bounds are used, the decision boundaries become more complex and (potentially) overlapped, and avoiding perturbing data during the initial stages of training can help the model's convergence, yielding  better models with a higher standard and adversarial accuracy.

Overall, this data shows that, in most scenarios, it is indeed beneficial to use an initial ST phase. Further, in all of the evaluated scenarios, there is at least one  optimal configuration that uses a mix of clean and adversarial examples during AT (i.e., \%AE$\neq$100) --- which suggests that AT is an important HP to optimize.  Further, across all scenarios, the fraction of Pareto optimal configurations that use a mix of clean and adversarial examples during AT is 82\%, and the optimal value of this parameter varies significantly across scenarios.

%the optimal configurations include when using only adversarial examples when training adversarially (i.e., \%AE=100), indicating that a combination of clean and perturbed inputs can yield better-quality models. 
%More in detail, the configurations that minimize the standard and adversarial error are found when pre-training the model using clean data and mixing clean and perturbed inputs.



%This implies that, for efficiency reasons, one cannot exclusively rely on AT.
%Since adversarial examples depend on the state of the model if we start generating adversarial examples using a random initialized (i.e, not trained) model, we misspend important resources.

%Further, it should be noted that this scenario corresponds to the lowest settings of the bound for that model and benchmark. When using larger bounds, we see more additional from using clean data trained model, since as the decision boundaries become more complex and (potentially) overlapped using a non-random initialized model when starting AT helps the model's convergence producing better models with a higher standard and adversarial accuracy.
%
%
%Furthermore, we also observe that the optimal configurations are not restricted when using only adversarial examples when training adversarially (i.e., \%AE=100), indicating that a combination of clean and perturbed inputs can yield better-quality models. 
%More in detail, the configurations that minimize the standard and adversarial error are found when pre-training the model using clean data and mixing clean and perturbed inputs.


In conclusion, these results show that, in order to maximize the efficiency and effectiveness of AT methods, it is important to appropriately tune both (i) the ratio of computational resources allocated to ST and AT (\%RAT) and (ii) the ratio of adversarial examples injected in a batch during AT (\%AE).


%that it might be beneficial both in terms of clean data and adversarial accuracy to divide the training into two phases: first, training the model with clean inputs and, second, training it using adversarial examples.
%Furthermore, the results suggest that both of these ratios need to be tuned and not selected a prior, which highlights the importance of tuning these parameters when performing HPO.


%As proofed in previous works~\cite{pgd,fgsm_fast,fgsm_free}, FGSM is not effective in training robust models when using larger bounds. However, since the same time was given to the training process, using FGSM allows training the models with more adversarial examples than PGD (computing the perturbation with PGD (using 20 iterations) is approx. 5$\times$ more expensive than FGSM) and thus yields  more accurate models. 

==> sections/6_HPO.tex <==

%Should clean and adversarial training share the same hyper-parameters?
%Should adversarial model hyper-parameters be tuned separately for clean and adversarial training?
%On the impact of sharing hyper-parameters in the clean and adversarial training phases?

%\section{Hyper-parameter tuning of clean and adversarial training phases}
%\vspace{-2mm}
\subsection{Should the HPs of ST and AT be tuned independently?} 
%\vspace{-1mm}
\label{sec:6_HPO}



%\section{Assuming 2 phases for training (clean followed by adv training), should we use the same hyper-parameters? What gains can we expect from tuning the hyper-parameters for each phase?}



%In the previous section, we concluded that there are gains when separating the training of a robust model into two phases (first, train using clean inputs and then perform AT) and tuning the parameters that control the percentage of clean and adversarial resources. 
%Thus, given these results, a new question arises that we aim at answering in this section: 


%\textcolor{red}{Several state-of-the-art works~\cite{delay_adv_train,inter_ST_AT} have pointed out the benefits of performing ST before AT. %in order to train models with comparable quality at a fraction of the cost.
%Thus, a new question arises that we aim at answering in this section: }
This section aims at answering the following question: 
given that the ST and AT phases share several HPs (e.g., batch size, learning rate, and momentum in the models considered in this study), how relevant is it to use different settings for these HPs in the two training phases? 
Note that, if we assume the existence of $C$ HPs in common between ST and AT, then enabling the use of different values for these HPs in each training stage causes a growth of the dimensionality of the HP space from $C$ to $2C$ (not accounting for any HP not in common) and, ultimately, to a significant increase in the cost/complexity of the HPT problem. Specifically, for the scenarios considered in this study, the cardinality of the HP space grows from 320 to 2560 distinct configurations. Hence, we argue that such a cost is practically justified only if it is counterbalanced by relevant gains in terms of error reduction.
%Given the two-phase training (clean followed by adversarial training), should the common HPs be used in both phases or tune those independently? 
%
%
To answer this question, we trained the models during 16 epochs and used different settings for the common HPs for ST and AT (Table~\ref{tab:fixed_hp}).
We consider three different settings (30\%, 50\%, and 70\%)\footnote[2]{We exclude the cases \%RAT=\{0,100\} in this study to focus on scenarios that contain both the ST and AT phases.} for the relative amount of resources (epochs) available for AT (\%RAT), as well as different settings of the perturbation bound $\epsilon$.% on the adversarial .
%We further consider the option suggested by Duesterwald et al.~\cite{hp_robust_ibm} of mixing clean and adversarial data during AT  by varying the percentage of adversarial examples while adversarially training the model (\%AE).



\begin{figure*}[t]
\centering
    %\captionsetup{justification=centering, font=small}
    \begin{subfigure}[b]{0.6\textwidth}
        \includegraphics[width=\textwidth]{plots/epochs_qualityHpLoss_barplot_legend.pdf}
    \end{subfigure}
    
    
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/imageNet/imageNet_epochs_qualityHpLoss_barplot_per.pdf}
        \caption{ResNet50/ImageNet}
        \label{fig:acc_red_imagenet}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/svhn/svhn_epochs_qualityHpLoss_barplot_per.pdf}
        \caption{ResNet18/SVHN}
        \label{fig:acc_red_svhn}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/cifar10/cifar10_epochs_qualityHpLoss_barplot_per.pdf}
        \caption{CNN/Cifar10}
        \label{fig:acc_red_cifar10}
    \end{subfigure}

    %\captionsetup{justification=justified}
    \caption{Reduction of the mean (in black), standard (in blue), and adversarial (in red)  error of the optimal configuration if the same or different hyper-parameters are used for the 2 phases of training using different scenarios and benchmarks.}
     \label{fig:acc_red}
     

%\end{figure*}

%\begin{figure*}[t]
%\centering
%    \captionsetup{justification=justified, font=small}
%    \begin{subfigure}[b]{0.6\textwidth}
%        \includegraphics[width=\textwidth]{plots/epochs_qualityHpLoss_barplot_legend.pdf}
%    \end{subfigure}

\vspace{3mm}
    %\captionsetup{justification=centering, font=small}
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=\textwidth]{plots/imageNet/imageNet_epochs_pgd_eps4.0_qualityHp_pdf.pdf}
        \caption{ResNet50/ImageNet}
        \label{fig:cdf_red_imageNet_pgd4}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=\textwidth]{plots/svhn/svhn_epochs_pgd_eps8.0_qualityHp_pdf.pdf}
        \caption{ResNet18/SVHN}
        \label{fig:cdf_red_svhn_pgd8}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=\textwidth]{plots/cifar10/cifar10_epochs_pgd_eps12.0_qualityHp_pdf.pdf}
        \caption{CNN/Cifar10}
        \label{fig:cdf_red_cifar10_pgd12}
    \end{subfigure}
    
    %\captionsetup{justification=justified}
    \caption{Cumulative distribution functions (CDFs) of the mean (in black),  standard (in blue), and adversarial  (in red) error reduction when using different HP settings for ST and AT w.r.t. the case in which common HPs are used in both phases. We use dashed and continuous lines to refer to different values of $\epsilon$.}% We plot CDF of the distribution of the ratio between the standard (or adversarial)  error if the same or different HPs are used.}
     \label{fig:cdf_acc_red1}
     %\vspace{-5mm}
\end{figure*}



%%
% Switch to:
% \% Error Reduction = (Error_same - Error_diff) / Error_same

%%% HP: <common_ST, common_AT, additional-AT-specific>
%%% Fig.1 : Err_same* <common_ST*, common_ST*, additional-AT-specific*>
%%%          Err_diff* <common_ST*, common_AT*, additional-AT-specific*> //NOTE: here common_ST*!=common_AT*

%** Fig.2: for each common HP, HP_i, and for each additional-AT-specific, ATS_i, and for each HP_j!=HP_i:
%              Err_same=  < HP_i, HP_i,ATS_i>
%              Err_dif=   < HP_i, HP_j,ATS_i>  // j!=i if this improves the "target" error, else j=i


%% Fig.3: (Err_AT_only*-Err_both_ST_AT_allowed*) / Err_AT_only*


We consider that the model's HPs can be optimized according to 3 criteria: i) clean data error (Error), ii) adversarial error (AdvError), and iii) the average of clean and adversarial error (MeanError). For each  of these 3 optimization criteria, \%RAT and bound $\epsilon$,  we report in Figure~\ref{fig:acc_red} the percentage of reduction of the target optimization metric for the optimal HP configuration obtained by allowing for (but not imposing) different settings of the  HPs in common to the ST and AT phases, with respect to the optimal HP configuration if one opts for using the same settings for the common HPs in both training phases, namely: 

\begin{equation}
    \text{\%Error Reduction} {\small=} 
    \frac{\text{Error}_{\text{same  HPs} } {\small-} \text{Error}_{\text{diff  HPs}}}{\text{Error}_{\text{same  HPs}}} \times 100 
\end{equation}

The results show that adopting different HP settings in the 2 phases can lead to significant error reductions for all the 3 optimization criteria. The peak gains extend up to approx. 30\% and are achieved for the case of ResNet18 with (relatively) large values of $\epsilon$ and when allocating a low percentage of  epochs  to AT (\%RAT=30\%). Overall,  the geometric means of the \% error reduction (across all models and settings of $\epsilon$ and \%RAT) is 9\%, 5\%, and 6\% for the Error, AdvError, and  MeanError criterion, respectively. 


%results geometric means, 
%imageNet 
%5.556264709324656
%8.72931560442094
%4.258782189857215


%cifar10
%2.1625961402981435
%6.4357605435479535
%2.0690963870264594

%svhn
%0.0
%9.367325252989364
%0.0


%The results obtained are reported in Figure~\ref{fig:acc_red} training a ResNet50 with ImageNet, ResNet18 with SVHN, and a CNN using Cifar10.
%For a given single-optimization objective (i.e., minimize error, or minimize adversarial error, or minimize the mean between standard and adversarial error), our findings show that there are always gains if one tunes the HPs of the two-phase training independently. 
%We observed a reduction of the (geometric) mean of the standard and adversarial error by up to 16\% and 7\%, respectively, while the peak gains are approximately 40\% .




Next, Figure~\ref{fig:cdf_acc_red1} provides a different perspective in order to quantify the benefits achieved by %performing a dedicated HPT to optimize the AT phase 
separately optimizing the HP of the AT phase (vs. using for the AT phase the same HPs settings in common with the ST phase), assuming to have executed an initial ST phase using any of the possible HPs settings. Specifically, we report the Cumulative Distribution Function (CDF) of the percentage of error reduction (for each of the 3 target optimization metrics), when allowing the use of the same or different common HP settings for the 2 phases and while varying the remaining (non-common) HPs, namely \%RAT, \%AE, and $\alpha$. 
%\textcolor{red}{
%More precisely, this analysis allows us to quantifying the impact of performing an additional phases of HPT to optimize the AT phase (and, thus, possibly use different settings for the HPs in common with the ST phase), once having
%that, for each HP settings in which the common HPs are set to be identical during AT and ST, 
%using independent settings for the common HP parameters when
%These results allow us to highlight that by independently tuning the HPs of the 2 training stages, the model's quality can be enhanced by up to approx. 5$\times$, 1.5$\times$, and 2.3$\times$, when minimizing the standard,  adversarial, or mean error, resp. 
These results allow us to highlight that by independently tuning the HPs of the 2 training stages, the model's quality is enhanced by up to approx. 80\%, 43\%, and 56\%, when minimizing the standard,  adversarial, or mean error, resp. 



\if0
\begin{figure*}[t]
\centering
    %\captionsetup{justification=justified, font=small}
    \begin{subfigure}[b]{0.6\textwidth}
        \includegraphics[width=\textwidth]{plots/epochs_qualityHpLoss_barplot_legend.pdf}
    \end{subfigure}

    
    \begin{subfigure}[b]{0.3\textwidth}
    \centering
        \includegraphics[width=\textwidth]{plots/imageNet/imageNet_epochs_pgd_eps4.0_qualityHp_pdf.pdf}
        \caption{ResNet50 ImageNet}
        \label{fig:cdf_red_imageNet_pgd4}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
    \centering
        \includegraphics[width=\textwidth]{plots/svhn/svhn_epochs_pgd_eps8.0_qualityHp_pdf.pdf}
        \caption{ResNet18 SVHN}
        \label{fig:cdf_red_svhn_pgd8}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
    \centering
        \includegraphics[width=\textwidth]{plots/cifar10/cifar10_epochs_pgd_eps12.0_qualityHp_pdf.pdf}
        \caption{CNN Cifar10}
        \label{fig:cdf_red_cifar10_pgd12}
    \end{subfigure}
    
    %\captionsetup{justification=justified}
    \caption{Cumulative distribution functions (CDFs) of the mean (in black),  standard (in blue), and adversarial  (in red) error reduction when using different HP settings for ST and AT w.r.t. the case in which common HPs are used in both phases. We use dashed and continuous lines to refer to different values of $\epsilon$.}% We plot CDF of the distribution of the ratio between the standard (or adversarial)  error if the same or different HPs are used.}
     \label{fig:cdf_acc_red1}
     %\vspace{-5mm}
\end{figure*}
\fi





Overall, these results may be justified by considering that the optimization objectives and constraints of the ST and AT phases are different, hence benefiting from using different HP settings. During ST, the training procedure focuses on maximizing standard accuracy, and the model's goal is to learn representations that generalize well to new data. 
In contrast, AT seeks to increase robustness against adversarial attacks, and the model needs to learn to differentiate between clean and perturbed examples correctly. Further, the AT phase benefits from a pre-trained model (using clean data), and, as such, this model is expected to require relatively small weight adjustments to defend against adversarial inputs. Thus, this phase is likely to benefit from more conservative settings of HPs such as learning rate and momentum than the initial ST, whose convergence could be accelerated via the use of more aggressive settings for the same HPs.
In fact, we confirmed this fact by analyzing the configurations that yield the 10 largest error reductions in Figure~\ref{fig:cdf_acc_red1}: better quality models used lower learning rates and batch sizes in the AT phase. 

%TODO: In fact, llooking at the configs that yield the 10 largest  error reductions in Fig.5, we have confirmed that this is the case.




Another factor that can justify the need for using different HP settings during ST and AT is related to the observation that the bound on the admissible perturbation ($\epsilon$) can have a deep impact on the model's performance, by exposing an inherent (and well-known~\cite{robustness}) trade-off: as the bound increases, the model may become more robust to adversarial inputs but at the cost of an increase in the  misclassification rate of clean inputs. To achieve an optimal trade-off between robustness and accuracy, it may be necessary to adjust the tuning of the HPs used during AT as $\epsilon$ varies, which in turn implies that the optimal HPs settings used during ST and AT can be different. 
In fact, by analyzing the results obtained on ResNet18/SVHN, for example, we see that the amplitude of the bound has an impact on the (adversarial) error reduction achievable by 
tuning independently the HPs of two phases of training: the 90$^{th}$ percentile of the percentage of clean error reduction is 50\% and 65\% using $\epsilon$=4 and $\epsilon$=8, respectively (see Fig.~\ref{fig:cdf_red_svhn_pgd8}).
%We conclude that in general optimizing the HPs of the two-phase training can always improve the quality of the final model.






\if0
\textcolor{red}{
Finally, we consider whether one can circumvent the need of tuning independently the (common) HPs for the ST and AT phases by simply avoiding to execute the ST phase, i.e., by simply performing AT. As mentioned in Section~\ref{sec:3_related_word}, a prior work~\cite{xxxx} had already noted advantages in having the AT preceded by an inital ST phase. However, unlike this prior work, our study also accounts for the possibility of using a mix of clean and adversarial data during AT --- which, at least hypotethically, may reduce the relevance of employing an initial training phases based solely on clean data.
%impact of  question has already been studied using different models, benchmarks, and HP configurations in other works~\cite{hp_robust_ibm,inter_ST_AT}, as mentioned in Section~\ref{sec:3_related_word}. 
%However, given that we are considering different experiments, we conduct a similar study. 
For each  optimization criterion,  we report in Figure~\ref{fig:acc_red_ratios} the \% of reduction of the target optimization metric when using both ST and AT (i.e., \%RAT$\leq$1) vs using exclusively AT (i.e., \%RAT=1)), i.e., 
%\vspace{-3mm}
\begin{equation}
  \text{\% Error Reduction} = \frac{\text{Error}_{\%RAT=1} - \text{Error}_{\%RAT\leq1}}{\text{Error}_{\%RAT=1}} \times 100.   %\vspace{-1mm}
\end{equation}
\textbf{TODO: what aobut the other hyper-parameters?}
The results show gains in standard, adversarial, and mean errors by up to approximately 23\%, 5\%, and 6\% respectively when ST is used before AT.  
Although our results are aligned with previous works, which concluded that performing ST before AT might yield better models), there is also a scenario (see Figure~\ref{fig:acc_red_cifar10_ratios}) where performing only AT can yield models with lower adversarial error and lower average of clean and adversarial error. 
Hence, these results highlight the importance of including in the HPT process the \%RAT.
}

\textbf{TODISCUSS: re-reading this part with a devil's advocate/reviewer perspective the results do not look super-convincing. Let's sleep over it but I am inclined to simply nuke this part.}


\begin{figure*}[t]
\centering
    %\captionsetup{justification=justified, font=small}
    \begin{subfigure}[b]{0.6\textwidth}
        \includegraphics[width=\textwidth]{plots/epochs_qualityHpLoss_barplot_legend.pdf}
    \end{subfigure}
    
    
    \begin{subfigure}[b]{0.27\textwidth}
        \includegraphics[width=\textwidth]{plots/imageNet/imageNet_epochs_2phases.pdf}
        \caption{ResNet50 ImageNet}
        \label{fig:acc_red_imagenet_ratios}
    \end{subfigure}
    \hspace{3mm}
    \begin{subfigure}[b]{0.27\textwidth}
        \includegraphics[width=\textwidth]{plots/svhn/svhn_epochs_2phases.pdf}
        \caption{ResNet18 SVHN}
        \label{fig:acc_red_svhn_ratios}
    \end{subfigure}
    \hspace{3mm}
    \begin{subfigure}[b]{0.27\textwidth}
        \includegraphics[width=\textwidth]{plots/cifar10/cifar10_epochs_2phases.pdf}
        \caption{CNN Cifar10}
        \label{fig:acc_red_cifar10_ratios}
    \end{subfigure}
    
    \caption{Standard, adversarial, and mean error reduction of the optimal configuration if ST is used or not before AT using different scenarios and benchmarks}
     \label{fig:acc_red_ratios}
\end{figure*}
\fi

%geometric mean
% svhn
%2.56170269863421
%19.6003733863814
%4.660562222634482
%imageNet
%4.147902475013908
%9.780893763135158
%0.9744201869147051
%cifaro
%0.0
%7.152514813862105
%0.0







%TODO: In fact, the data on svhn shows that the amplitude of the bound has an impact on the (adv.) error reduction achievable by tuning indepentently the HP of adv. and clean training: the 90-th percentile of clean error reduction with eps=4 is 1.67 vs 2. for eps=8 ... what about adversarial


%Moreover, the magnitude of the perturbation used during adversarial training can significantly impact the model's performance. As the bound increases, the model may become more robust but may also start to misclassify clean examples. Hence, it is crucial to find the right trade-off between robustness and accuracy, which may require tuning the HPs independently for each training phase.



%Therefore, it is expectab can lead to different settings for the corresponding HPs.
%Moreover, the magnitude of the perturbation used during adversarial training can significantly impact the model's performance. As the bound increases, the model may become more robust but may also start to misclassify clean examples. Hence, it is crucial to find the right trade-off between robustness and accuracy, which may require tuning the HPs independently for each training phase.



%
%varied from approximately 7.5\% to 18\% for ResNet50 using ImageNet, while the adversarial accuracy reduction ranged from around 2.5\% to 15\%.
%Considering the ResNet50 and ImageNet benchmark, accuracy reduction varies from approximately 7.5\% to 20\%, and the adversarial accuracy reduction varies from around 2.5\% to 15\%. 
%Similar reductions were obtained when training a CNN using Cifar10. \textbf{update info}
%, by carefully tuning the HPs of both training phases, even considering a single-objective optimization, we are able to improve both standard and adversarial accuracy at the same time.
\if 0

Interestingly, the larger gains attained by using different HPs occur when models are trained with less adversarial data. In other words, the use of distinct HP settings for the clean and adversarial training phases leads to larger error reductions  when fewer adversarial examples are fed to the model. This is particularly noticeable when training ResNet50 with ImageNet (Figure~\ref{fig:acc_red_imagenet}). 
Overall, these experimental data highlight the importance of selecting appropriate HPs for training robust machine learning models.


Next, Figure~\ref{fig:acc_red1}  reports the clean data and adversarial error  reduction for a set of configurations composed of the common HPs in the 2 phases whether we use different or the same HPs for both training phases (and selecting the best ones for the non-common adversarial HPs). 
We consider two cases where we optimize for standard and adversarial error. The results show that, regardless of the optimization goal, all configurations achieved better quality when the HPs of the two training phases are tuned independently. Training a ResNet50 ImageNet, ResNet18 SVHN, and a CNN Cifar10, the standard error reductions when using the same or different HPs ranged mainly from 5\% to 20\%, and the adversarial error reductions are around 7\%, while the peak gains are approximately 80\%.
\fi







%\input{plots/tables.tex}




==> sections/7_multiBudgets.tex <==



%\section{Hyper-parameter Optimization for adversarial training}
%\vspace{-2mm}
\subsection{Can cheap AT methods be leveraged to accelerate HPT?}
%\vspace{-1mm}
% Can information on cheap adversarial training methods be used to inform expensive and more robust methods?
\label{sec:7_multiBudgets}

\input{plots/correlations}

So far, we have shown that in adversarial settings the complexity of the HPT problem is exacerbated due to the need for optimizing a larger HP space. 
In this section, we show that, fortunately, AT provides also new opportunities to reduce the HPT cost. % for adversarially robust models.
%
Specifically, we propose and evaluate a novel idea: leveraging alternative AT methods, which impose lower computational costs but provide weaker robustness guarantees to sample HP configurations in a cheap, yet informative, way. As discussed in Section~\ref{sec:3_related_word}, PGD is an iterative method, where each iteration refines the perturbation with the objective of maximizing loss. Hence, a straightforward way to reduce its cost (at the expense of robustness) is to reduce the number of executed iterations. We also note that the computational cost of FGSM is equivalent to that of a single PGD iteration. 






\if0
\begin{table*}[t]
\centering
\begin{tabular}{ c|c } 
\textbf{Fidelities}  &\textbf{Values} \\\hline \hline
No. of Iterations &  \{FGSM, PGD5, PGD10, PGD20\} \\ \hline
Epochs & \{ 1,2,4,8,16  \} \\[2mm]
\end{tabular}
\caption{Fidelities (budgets) considered}
\label{tab:budgets}
\end{table*}
\fi



\if 0
The previous studies emphasize the importance of HP tuning when training a robust model. Consequently, it is fundamental to extend current HP optimizers to incorporate At. 
Nonetheless, additional problems  that need to be addressed are inherited from AT limitations.
One such issue is the increased number of HPs to tune, which for example hinders the adoption of optimizers that rely on costly methods such as Bayesian Optimization (BO) due to their high computational cost and slower convergence when large search spaces are considered. 
Moreover, recent state-of-the-art solutions have aimed to reduce the optimization cost by exploiting cheap, low-fidelity models (e.g., trained with a fraction of the available data) to extrapolate the quality of fully trained models.
Therefore, due to the high cost of PGD method, one might want to use FGSM or PGD with a small number of iterations as a new fidelity in order to reduce the cost of identifying optimal configurations using PGD. Thus, a new question arises: Can the information on HP tuning collected with cheap methods (e.g., FGSM) be used to gather knowledge on expensive methods (PGD)?


%Due to time and resource constraints, the next studies were only conducted using a ResNet50 with ImageNet, which corresponds to the most complex and largest model and biggest dataset considered in the various experiments that we conducted. 



PGD has been shown to yield models with better robustness when larger bounds are used \cite{pgd,fgsm_fast,fgsm2} compared to FGSM. However, when smaller bounds for the attack are considered, FGSM and PGD yield models with similar quality (both in terms of standard and adversarial accuracy), but at a fraction of the time.

\fi



We build on these observations to propose incorporating the number of PGD iterations as an additional fidelity dimension in multi-fidelity HPT optimizers, such as taKG~\cite{takg}. %(see Section~\ref{sec:3_related_word}). 
We choose to test the proposed idea with taKG since this technique supports the use of an arbitrary number of fidelity dimensions (e.g., dataset size and number of epochs) and determines how to explore the multi-dimensional fidelity via black-box modeling techniques (see Section~\ref{subsec:HPT}). 
%

In order to assess the soundness and limitations of the proposed approach, we first analyze the correlation of the standard and adversarial error between HP configurations that use PGD with 20 iterations (which we consider as the maximum-fidelity/full budget) vs.~PGD with 10 and 5 iterations and FGSM (which, as already mentioned, is computationally equivalent to 1 iteration of PGD). In Figure~\ref{fig:correlation},  we observe that the correlation varies for different bounds on adversarial perturbations across the considered models/datasets. 
We omit the correlation for ResNet50/ImageNet using $\epsilon$=4 since the results are very similar to $\epsilon$=2.
The scatter plots  clearly show the existence of a very strong correlation (above 95\%) for all the considered methods for ResNet50/ImageNet and for all the considered bounds. For ResNet18/SVHN and CNN/Cifar10, the correlation of PGD 5 and 10 iterations remains quite strong (always above 80\% and typically above 90\%), whereas lower correlations (as low as 53\%) can be observed for FGSM, especially when considering adversarial error and larger values of $\epsilon$ . This is expected, as previous works~\cite{fgsm2,catastrophic_overfitting} had indeed observed that FGSM tends to be less robust than PGD when larger $\epsilon$ values are used (being subject to issues such as catastrophic-overfitting that lead to a sudden drop of adversarial accuracy). Still, even for FGSM, the correlation is always above 90\% with CNN/Cifar10 and is relatively high (around 70\%) also with ResNet18/SVHN for the smaller considered bound ($\epsilon=4$).% Figures~\ref{fig:correlation_acc_svhn_4} and \ref{fig:correlation_advacc_svhn_4}).





%visualize the strong correlation between the different methods considered. Moreover, we also report the coefficient of correlation between the different methods, which is normally large (close to 1), and proves the high correlation between these methods.

%Figure~\ref{fig:correlation} reports the correlation of the standard and adversarial error between PGD with 20 iterations (that we consider high-fidelity/full budget) and FGSM, PGD with 5 and 10 iterations considering different $\epsilon$ when training  a ResNet50 with ImageNet, a ResNet18 with SVHN, and CNN with Cifar10.
%models and benchmarks. In this case, we include a CNN using MNIST, since due to its lower training cost, we were able to train the model using more bounds and point different results when larger bounds are used. 
%Hence, it is easy to visualize the strong correlation between the different methods considered. Moreover, we also report the coefficient of correlation between the different methods, which is normally large (close to 1) and proves the high correlation between these methods.
%As expected, when smaller values of $\epsilon$ are considered both FGSM and PGD present similar performance and a strong correlation.
%However, when training with larger bounds, %(e.g., a CNN with MNIST and $\epsilon > 0.3$ (see Figure~\ref{fig:bound_acc_mnist})w, 
%we verify a reduction in the quality of FGSM's trained models and a decrease in the correlation between FGSM and PGD  when $\epsilon$ increases.











%These conclusions are corroborated by the results present in Figure~\ref{fig:correlation2} which reports the correlation of the standard and adversarial error between FGSM and PGD (20 iterations) for a set of configurations using different bounds when training the previous models and benchmarks. 
%We considered FGSM and PGD with 5, 10, and 20 iterations. Based on this figure, 
%These results strengthen the idea of exploiting cheap adversarial algorithms (i.e., FGSM, PGD5, and PGD10) to gather knowledge and extrapolate it on expensive methods (PGD20).




We also report, in Figure~\ref{fig:cost_imageNet}, %and \ref{fig:cost_cifar10}
 %reports,
 the CDF of the training time reduction using FGSM, PGD with 5 and 10 iterations, and ST w.r.t.~PGD20 for ResNet50/ImageNet. %with 20 iterations 
 % and CNN Cifar10, respectively.
The CDFs show that the training time reductions for a given AT method vary since the ratio of computed adversarial examples  depends on the \%RAT and \%AE parameters. Overall, the maximum (median) training time reduction is approx. 
%5.7$\times$ (2.2$\times$), 2.8$\times$ (1.9$\times$), 1.8$\times$ (1.5$\times$), and 7$\times$ (2.3$\times$), 
83\% (54\%), 66\% (42\%), 47\% (28\%), and 86\% (53\%)
for FGSM, PGD5, PGD10, and STD, compared to PGD20, which confirms that leveraging these ``cheap'' surrogate methods can significantly reduce the cost of testing HP configurations.




\begin{figure*}[t]
\centering
    %\captionsetup{justification=centering, font=small}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[ width=\textwidth]{plots/imageNet/resnet_imagenet_Cost_Loss.pdf}
        \caption{ResNet50/ImageNet $\epsilon$\textdblhyphen2}
        \label{fig:opt_imageNet}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[ width=\textwidth]{plots/svhn/resnet_svhn_Cost_Loss.pdf}
        \caption{ResNet18/SVHN $\epsilon$\textdblhyphen8}
        \label{fig:opt_svhn}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/cifar10/cnn_cifar10_Cost_Loss.pdf}
        \caption{CNN/Cifar10 $\epsilon$\textdblhyphen12}
        \label{fig:opt_cifar10}
    \end{subfigure}
    
    %\captionsetup{justification=justified}
    \caption{Average standard and adversarial error using different optimizers.}
     \label{fig:optimizers}
\end{figure*}




%Although the reduction of training depends on the AT method as well as the \%RAT and \%AE, we clearly see a reduction in the training times. The training time is reduced on average by 2.5, 1.8, 1.4, and 2.6 using FGSM, PGD5, PGD10, and STD compared to PGD20. Moreover, as expected, these reductions are larger with FGSM and standard training.


%gsm average 2.4491229941271624
%pgd5 average 1.7840436220902043
%pgd10 average 1.3932490313416133
%pgd20 average 2.6009418430412152

%Add something short where you highlight that the cost reduction depend on the method, as as well as rat and ae... but that they can be up to xxx times when using fgsm and that on AVG for each method are xxx yyy zzz


%\section{HTP for Adversarially Robust Models}
%\label{sec:hpo_at}

Supported by these findings, we evaluate our proposal by integrating the number of PGD iterations as an additional fidelity dimension in taKG~\cite{takg}. As discussed in  Section~\ref{sec:3_related_word}, taKG is a HPT method that natively supports the use of multiple fidelity types, which we refer to as fidelity dimensions, e.g., number of epochs, input size, and dataset size. 
%
%In light of the results of the previous section, we consider as  HP space for this study one in which the HPs of the ST and AT phases are independently optimized (which yields a total of 9 HPs). 
Based on the results of the previous section, we independently optimize the HPs of the ST and AT phases, which yields a search space composed of a total of 9 HPs (Table~\ref{tab:fixed_hp}). 
The following multi-fidelity solutions are compared:

\begin{itemize}
%\noindent $\bullet$ 
\item \textit{taKG (epochs, PGD iter)}: the proposed solution, which uses taKG as the underlying HPT method and employs as fidelity the number of epochs and %the number 
of PGD iterations. We discretize these 2 dimensions (Table~\ref{tab:budgets}). 
%\noindent $\bullet$  
\item \textit{taKG (epochs)}: taKG  using as fidelity only the number of epochs. 
%\noindent $\bullet$ 
\item \textit{taKG (PGD iter)}: taKG using  as fidelity only the number of PGD iterations.
%\noindent $\bullet$  
\item \textit{HB (epochs)}: HyperBand~\cite{hyperband}, a popular (single-dimensional) multi-fidelity optimizer, which uses  the number of epochs as fidelity.
\end{itemize}

We further compare against BO using EI as acquisition function and Random Search (RS). These optimizers only perform high-fidelity evaluations.
The evaluation of these alternative solutions is performed by exploiting the dataset already described in Section~\ref{sec:experiment}, which specifies the model quality (error and adversarial error) for all possible HPs, $\epsilon$ and fidelity settings reported in Tables~\ref{tab:fixed_hp},~\ref{tab:bounds} and \ref{tab:budgets}. 



%conduct a study using the previously collected data where we benchmark several optimizers to perform HP tuning of the two-phase training. 
%Moreover, we proposed the usage of FGSM and PGD iterations as additional fidelity. 
%Since taKG is the only optimizer that allows using several budgets at the same time, we benchmark it using as budgets this additional dimension (i.e., PGD iterations) and epochs. 
%We compared it with HyperBand, a commonly used multi-fidelity HPT optimizer, but we only used the number of epochs as the budget. We further compared against BO with EI and Random Search which only permits high-fidelity evaluations. 







We define the optimization problem as follows: %\vspace{-1.5mm} 
\begin{equation}
    \underset{x}{\min} \text{ } \lambda \cdot \text{Error}(x,s{\small =}1) + (1{\small -}\lambda) \cdot \text{Adv.Error}(x,s{\small =}1) %\vspace{-1.5mm}
\end{equation} 
where $x$ is a vector defining the HPs, $s$ is a vector that encodes the ratio of budget allocated for each fidelity dimension, and $\lambda$ is a weight factor that we set to 0.5 to equally balance the standard and adversarial errors. For a fair comparison, when a single fidelity dimension (e.g., epochs) is used, we set the other fidelity dimension (e.g., PGD iterations)  to its maximum value. % (e.g., when using PGD iterations as the budget, we set the number of epochs to its maximum value).
%The values of the fidelities considered are reported in Table~\ref{tab:budgets}. 
%
We run each optimizer using 20 independent seeds. We set the bound $\epsilon$ to 2, 8, and 12 to optimize ResNet50/ ImageNet, ResNet18/SVHN, and CNN/Cifar10. 
Based on Figure~\ref{fig:correlation}, the 3 settings correspond to scenarios with relatively high, low, and medium correlation for the budget dimension defined by PGD iterations, resp.










Figure~\ref{fig:optimizers} reports the  average and standard deviation of the optimization goal (i.e., $0.5\cdot\text{Error} + 0.5\cdot\text{Adv.Error}$) as a function of the optimization time for the different HPT optimizers and different models/datasets.
%
The results show that the proposed solution, which adopts PGD iterations as extra fidelity along with the number of epochs (taKG - epochs \& PGD iter), clearly outperforms all the alternative solutions in ResNet50/ImageNet and ResNet18/SVHN. 
%
%
The largest gains can be observed with ResNet18/SVHN (Fig.~\ref{fig:opt_svhn}). Here, at the end of the optimization process, the proposed solution identifies a configuration of the same quality as the ones suggested by the other baselines, namely taKG - epochs, HB, BO-EI, by achieving speed-ups of 2.1$\times$, 3.7$\times$, and 5.4$\times$, respectively.
%
Using the same metric (time spent to recommend a configuration of the same quality as the ones suggested by the other optimizers at the end of the optimization process) with ResNet50/ImageNet, the proposed solutions achieve slightly smaller, but still significant speed-ups, namely 1.28$\times$, 1.97$\times$ and 2.45$\times$ w.r.t.~taKG - epochs, HB, BO-EI. Interestingly, with ResNet50/ImageNet the proposed solution provides solid speed-ups also during the first stage of the optimization. Specifically, if we analyze the first half of the optimization process  (corresponding to approx. 83 hours (see Figure~\ref{fig:opt_imageNet})) the proposed solution identifies configurations of the same quality as taKG - epochs, HB, BO-EI, with speed-ups of 1.7$\times$, 2$\times$ and 2.6$\times$, respectively.



%{achieving time reductions of 1.5$\times$ and 2.3$\times$ compared to the same optimizer using just number of epochs or PGD iterations, resp.}. The gains are larger for the case of ResNet50 ImageNet (Figure~\ref{fig:opt_imageNet}), which is expected, given that as shown in Figure~\ref{fig:correlation}, this is the scenario that exhibits the highest correlation across different settings of PGD iterations. It is, however, worth noting that noticeable gains can be achieved also with ResNet18 SVHN (Figure~\ref{fig:opt_svhn}), which showed a relatively low correlation (around 60\%) for FGSM.
%
With CNN Cifar10 (Figure~\ref{fig:opt_cifar10}), the proposed approach remains the best-performing solution, although with smaller gains when compared to taKG with epochs. Still, the proposed solution can identify configurations with the same quality as the best alternative (taKG epochs) by saving approx.~40\% of the time (i.e., in 22 hours vs. 32 hours). We argue that the gains with CNN Cifar10 are relatively lower than in the other scenarios considered in Figure~\ref{fig:optimizers} since  those models are larger and more complex. As such, they benefit more from the cost reduction opportunities provided by using a reduced number of PGD iterations.

We also observe that the exclusive use of  PGD iterations with taKG yields worse performance than using solely number of epochs. This is not surprising, given that number of epochs is arguably one of the most direct ways of controlling the cost of configuration sampling and is, indeed, among the most commonly adopted budgets in multi-fidelity optimizers~\cite{fabolas,hyperband,hyperjump}. %Overall, 
This result confirms that PGD iterations represent a valuable mean to accelerate multi-fidelity HPT optimizers to train robust models and that it complements, but does not replace, "conventional" budget settings like number of epochs or dataset size.

\if 0
\textcolor{red}{
Finally, our approach reduces the optimization time by up to 2$\times$, 2.4$\times$, and 3$\times$ compared to HB,  BO-EI and RS, resp. 
The comparison with the last 2 optimizers confirms the superiority  of multi-fidelity methods. While this is not  a novel result~\cite{hyperjump}, it highlights the relevance of developing novel approaches, like the one proposed here, to advance state-of-the-art multi-fidelity HPT techniques.
%The comparison with BO-EI and Random Search (which, recall, only use high-fidelity evaluations) confirms, also in the scenarios considered in this work, the superiority  of multi-fidelity HPT techniques. While this is not  a novel result~\cite{hyperjump,trimtuner,hyperband}, it highlights the relevance of developing novel approaches, like the one proposed here, to advance state-of-the-art multi-fidelity HPT techniques.
}
\fi

%time reductions of takg both
% imageNet
% -to 0.33xtotal_time
%     - 1.5 takg epochs
%     - 2.3 takg pgd
%     - 2.0 hb
%     - 2.4 ei
%     - 3.0 rand
    
% -to 0.66xtotal_time
%     - 1.2 takg epochs

% SVNH
% -to 0.33xtotal_time
%     - 2.2 takg epochs

% Cifar10
% -to 0.33xtotal_time
%     - 0.95 takg epochs
%     - 1.84 takg pgd
%     - 2.0 hb
    
% -to 0.66xtotal_time
%     - 1.22 takg epochs



%, while being on par with the versio

%esults obtained for the different HPT optimizers to perform HPT while training a robust model using a ResNet50 with ImageNet, a ResNet18 with SVHN, and a CNN with Cifar10. We plot .
%For a given maximum optimization time (corresponding to the final time reported in the plots of Figure~\ref{fig:optimizers}), taKG using as fidelities the number of epochs and PGD iterations reduces the error by up to 1.3\%, 4.3\%, and 3\% compared to taKG using just the number of epochs, or just PGD iterations, and HB, respectively. 
%When compared to BO with EI and Random Search which only use high-fidelity evaluations, this error reduction increases to 4.5\% and 7\%, respectively.   
%Moreover, the joint usage of the number of epochs and PGD iterations as fidelities speeds up the optimization time with respect to the baselines to recommend optimal configurations. This means that taKG using these to budgets can recommend better configurations in a fraction of the time. This is particularly notorious when training larger models such as ResNet50 with ImageNet and ResNet18 with SVHN (see Figures~\ref{fig:opt_imageNet} and \ref{fig:opt_svhn}), where the additional budget allows us to reduce more significantly the cost of evaluating configurations. 





%Consider that cheap methods are FGSM or PGD with a small number of iterations and clean data training.
%A precondition for this question: cheap methods must yield worse (adv.) accuracy than expensive ones.
%Here, for a fair comparison, we ensure that the same amount of data/inputs are used to train the models (that means in the next experiments we used as the stop condition the number of epochs to train the models).

%We see that when we use "acceptable" bounds (i.e., bounds that allow training a robust model with both methods), we see a strong correlation both in the standard and adversarial accuracy between FGSM and PGD. 






\if0

\input{plots/correlation.tex}


\newpage
\subsection{CIFAR10 (stop condition epochs)}
\input{plots/cifar10_epochs}

\subsection{CIFAR10 (stop condition epochs with early stopping)}
\input{plots/cifar10_epochs_earlyStop.tex}



\subsection{MNIST (stop condition epochs)}
\input{plots/mnist_epochs}

\subsection{MNIST (stop condition epochs with early stopping)}
\input{plots/mnist_epochs_earlyStop.tex}


\subsection{SVHN (stop condition epochs)}
TODO
%\input{svhn_epochs}

\subsection{ImageNet (stop condition epochs)}
\input{plots/imageNet_epochs}

\subsection{ImageNet (stop condition epochs with early stopping)}
\input{plots/imageNet_epochs_earlyStop.tex}
\fi

==> sections/8_conclusion.tex <==

%\vspace{-1mm}
\section{Conclusions and Future work}
\label{sec:8_conclusion}
%\vspace{-1mm}



This paper focused on the problem of HPT for robust models. By means of an extensive experimental study, we first quantified  the relevance of  %selecting the ratio of computational resources allocated to a preliminary clean data training, as well as the ratio of adversarial examples to use in the AT phase. We also 
independently tuning  the HPs used during standard and adversarial training.
%
%conducted an empirical study to show that adversarial training should be preceded by an initial clean data training phase and that the hyper-parameters of these two training phases (clean follow by adversarial) should be tuned independently in order to obtain models with better quality.
%
We then proposed and evaluated a novel fidelity dimension that becomes available in the context of AT. Specifically, we have shown that cheaper AT methods can be used to obtain inexpensive estimations of the quality achievable via expensive state-of-the-art AT methods and that this information can be effectively exploited to accelerate HPT. 
We extended taKG, a state-of-the-art HPT method, by incorporating  the PGD iterations as an additional fidelity dimension (along with the number of epochs) and achieved cost reductions by up to 2.1$\times$.

It is worth noting that the idea of employing ``cheap'' AT methods as proxies to estimate the quality of HP configurations with more robust/expensive methods is generic, in the sense that it can be applied, at least theoretically, to any multi-fidelity optimizer. As part of our future work, we plan to integrate this novel approach in a new HPT framework, specifically designed to cope with adversarially robust models.

%In future work, we intend to investigate the possibility of using ``cheap'' AT methods (like PGD) as proxy to d

%approach can be applied to any multi-fidelity optimizer and as future work, we plan to integrate this additional fidelity dimension with other multi-fidelity HP optimizers.
%}

%\textcolor{red}{TODO: 1. Integrated with taKG. Short summary of results. 2. It is worth noting that the proposed \textbf{approach} can be applied to any multi-fidelity optimizer and as future work, we plan to integrate these  additional fidelity dimensions with other multi-fidelity HP optimizers.}

% (by extending, taKG, a recent multi-fidelity technique).



%Moreover, we extended several multi- and high-fidelity HPT optimizers to the adversarial setting, where we proposed the usage of PGD iterations as an additional fidelity to reduce the optimization cost.
%This fidelity can speed up the optimization process and reduce the error of the recommended configuration.
